GADGET: Online Resource Optimization for Scheduling Ring-All-Reduce Learning Jobs

Fueled by advances in distributed deep learning (DDL), recent years have witnessed a rapidly growing demand for resource-intensive distributed/parallel computing to process DDL computing jobs. To resolve network communication bottleneck and load balancing issues in distributed computing, the so-called ``ring-all-reduce'' decentralized architecture has been increasingly adopted to remove the need for dedicated parameter servers. To date, however, there remains a lack of theoretical understanding on how to design resource optimization algorithms for efficiently scheduling ring-all-reduce DDL jobs in computing clusters. This motivates us to fill this gap by proposing a series of new resource scheduling designs for ring-all-reduce DDL jobs. Our contributions in this paper are three-fold: i) We propose a new resource scheduling analytical model for ring-all-reduce deep learning, which covers a wide range of objectives in DDL performance optimization (e.g., excessive training avoidance, energy efficiency, fairness); ii) Based on the proposed performance analytical model, we develop an efficient resource scheduling algorithm called GADGET (greedy ring-all-reduce distributed graph embedding technique), which enjoys a provable strong performance guarantee; iii) We conduct extensive trace-driven experiments to demonstrate the effectiveness of the GADGET approach and its superiority over the state of the art.

==> AllReduce_Scheduling_INFOCOM'21/Abstract/Abstract.tex <==
% !TEX root = ../AllReduce-Scheduling-INFOCOM'21.tex

\begin{abstract}
Fueled by advances in distributed deep learning (DDL), recent years have witnessed a rapidly growing demand for resource-intensive distributed/parallel computing to process DDL computing jobs.
To resolve network communication bottleneck and load balancing issues in distributed computing, the so-called ``ring-all-reduce'' decentralized architecture has been increasingly adopted to remove the need for dedicated parameter servers.
To date, however, there remains a lack of theoretical understanding on how to design resource optimization algorithms for efficiently scheduling ring-all-reduce DDL jobs in computing clusters.
This motivates us to fill this gap by proposing a series of new resource scheduling designs for ring-all-reduce DDL jobs.
Our contributions in this paper are three-fold:
i) We propose a new resource scheduling analytical model for ring-all-reduce deep learning, which covers a wide range of objectives in DDL performance optimization (e.g., excessive training avoidance, energy efficiency, fairness);
ii) Based on the proposed performance analytical model, we develop an efficient resource scheduling algorithm called GADGET (\underline{g}reedy ring-\underline{a}ll-reduce \underline{d}istributed \underline{g}raph \underline{e}mbedding \underline{t}echnique), which enjoys a provable strong performance guarantee;
iii) We conduct extensive trace-driven experiments to demonstrate the effectiveness of the GADGET approach and its superiority over the state of the art.
\end{abstract}

==> AllReduce_Scheduling_INFOCOM'21/Sec1-Intro/Sec1-Intro.tex <==
% !TEX root = ../AllReduce-Scheduling-INFOCOM'21.tex

\section{Introduction} \label{sec:intro}

%Paragraph1: Background and introduce the ring-all-reduce architecture
In recent years, the rise of complex deep learning applications has led to a rapidly growing demand for resource-intensive (e.g., GPUs, memory, energy) distributed/parallel computing to process deep learning training tasks.
%Indeed, the recent success of deep learning is attributed in large part to the advances in multi-core GPU technologies (on the micro chip scale) and networked computing cluster technologies (on the macro data center level), which facilitates the development of highly parallel and distributed deep learning (DDL) training.
%DDL frameworks include TensorFlow\cite{??}, PyTorch\cite{??}, MXNet\cite{???}, etc.
Traditionally, most distributed deep learning (DDL) frameworks are based on the parameter server (PS)-worker architecture, which consists of a set of PS(s) and workers. 
%PSs serve as the global memory that stores the deep learning model parameters, while the workers share the same copy of the deep learning model and compute gradients to update the global model parameters at the PSs.
Despite its simplicity, the PS-worker architecture suffers from two scalability limitations:
i) The topology of the PS-worker architecture creates a {\em communication bottleneck} at each PS as the number of workers increases; and
ii) The centralized PSs are vulnerable to the {\em single-point-of-failure risk}.
To overcome these scalability weaknesses, the more sophisticated {\em ``ring-all-reduce''} (RAR) parallel computing architecture has become increasingly popular for DDL training and has been supported by many mainstream DDL frameworks (e.g., Tensorflow~\cite{Abadi16:TensorFlow}, Pytorch~\cite{Paszke19:Pytorch}).
Specifically, by forming a ring between the workers to jointly perform parameter sharing and reduction, the RAR  architecture removes the need for dedicated PS(s), hence alleviating the single point of failure. %the communication bottleneck and single point of failure.
%Moreover, it has been shown that the RAR architecture is bandwidth-optimal with the assumption that the all-reduce tensor (i.e., gradients to be aggregated or averaged) is large enough~\cite{Patarasuk09:Ring-AllReduce} (i.e., the amount of exchanged information under RAR is asymptotically independent of the number of workers; see Section~\ref{sec:Preliminaries} for further details).
%is asymptotically {\em bandwidth-optimal}~\cite{Patarasuk09:Ring-AllReduce} (i.e., the amount of exchanged information under RAR is asymptotically independent of the number of workers; see Section~\ref{sec:Preliminaries} for details).


%Paragraph 2: Argue that it remains to consider resource scheduling and optimization for 
However, with the increasing adoption of the RAR architecture for DDL training, an important question naturally emerges: {\em How could we design %computing 
resource optimization algorithms to efficiently schedule RAR-based DDL training jobs over networked computing clusters?}
Answering this question is critical because:
i) Multi-core high-throughput GPU hardware for cloud-based machine learning services is expensive, which requires efficient GPU utilization.
For example, an Amazon EC2 eight-core GPU instance with NVLink connection costs more than \$31 per hour\cite{P3_COST:2021};
%The limited and expensive GPU resources require efficient GPU utilization;
%ii) Although each individual RAR-based DDL training job is bandwidth-efficient, multiple RAR-based DDL training jobs have to share and compete for the computation and communication resources in a {\em networked} computing cluster.
ii) Due to the resource competition among multiple RAR-based DDL training jobs in the cluster,
if scheduling is not done strategically, DDL training jobs could suffer from large latency;
and iii) RAR-based DDL jobs are often trained by variants of the {\em iterative} stochastic gradient descent (SGD) method to optimize thousands or even millions of parameters. 
Their completion times are defined by the convergence processes of these SGD-based methods, which often exhibit the {\em ``diminishing return effect''} in terms of the gains in training accuracy as the number of iterations increases.
%are highly dependent on the learning models/hyperparameters (i.e., neural network architectures, step-sizes/learning rates) and 
For instance, it has been shown in \cite{Jeon2018:multi-tenant} that approximately 75\% of DDL jobs reach within 0.1\% of the lowest training loss using only 40\% of the epochs.
Allocating too many computing resources to one job not only induces high GPU and energy costs as well as unfairness to other DDL jobs, but also leads to unnecessary training time with little learning accuracy performance gain in return.

However, optimizing scheduling and resource allocation for RAR-based DDL is highly non-trivial due to several technical challenges.
{\em First}, the hop-by-hop dependence in the ring structure renders the placement of workers highly sensitive to intra- and inter-server communications, decided by the underlying computing network topology.
Also, as will be shown later, the ring topology violates the loop-less assumption of many existing algorithms for virtual computing resource allocation problems \cite{Rost18:VNE, Avin18:CoRR, Rost19:Sigcomm}, which necessitates new algorithmic design techniques.
{\em Second}, the %computing 
%and cover-type (due to QoS guarantee)
resource allocation for each RAR-based DDL job is subject to packing-type constraints (due to resource limits), which implies NP-Hardness.
{\em Lastly}, the scheduler is not aware of DDL job arrivals beforehand, which calls for {\em online} optimization algorithm design.
Perhaps due to these challenges, to date, results on scheduling and resource allocation for RAR-based DDL training remain limited.
This motivates us to fill this gap by proposing an efficient resource scheduling algorithm called GADGET (\underline{g}reedy ring-\underline{a}ll-reduce \underline{d}istributed \underline{g}raph \underline{e}mbedding \underline{t}echnique), which addresses the aforementioned technical challenges with strong theoretical performance guarantees.
%and offer strong theoretical performance guarantees. 
The main results in this paper and their significance are summarized as follows:

\begin{list}{\labelitemi}{\leftmargin=1em \itemindent=0em \itemsep=.2em}

\item By extracting the key architectural features of RAR-based DDL training jobs, we develop a new analytical model for scheduling RAR-based DDL jobs over networked environments.
Based on this model, we formulate a general online performance optimization framework for RAR-based DDL training.
%, which covers a wide range of objectives (e.g., excessive training avoidance, energy consumption minimization, fairness between RAR-based DDL jobs).
We note that, due to the heterogeneous internal (i.e., between containers in the same physical server) and external (i.e., between physical machines within or beyond the same rack) communications, the resource scheduling and allocation problem for RAR-based DDL training is far more challenging than those for the PS-worker architecture.

\item To address the new challenges arising from RAR-based DDL training, we develop an efficient GADGET algorithm that can provide provably strong performance guarantee.
Our GADGET approach is based on a ``divide-and-conquer'' approach.
Specifically, we first show that the formulated RAR-based training scheduling problem over the temporal domain possesses a submodular structure due to its partition matroid nature, and hence can be decomposed in the temporal domain and solved by a greedy approach with worst-case approximation ratio guarantee.

\item Next, we focus on the decomposed subproblem in each time-slot, which remains NP-Hard due to the packing-type constraints.
We note that the ring-structure of RAR-based DDL jobs renders existing methods ineffective.
To address this challenge, we propose a {\em generalized} virtual graph embedding (G-VNE) technique that guarantees a $\frac{1}{3\Gamma}$-fraction of the maximum utility value, where $\Gamma \geq 1$ is a problem-dependent constant.
Combining this with the submodular property implies that GADGET achieves an $\frac{1}{3\Gamma+1}$ overall competitive ratio.


\item Lastly, we conduct experiments to examine the performance of our GADGET algorithm.
%with a variety of RAR-based DDL models.
We demonstrate the good approximation ratio of G-VNE, which is the main component of GADGET algorithm by using real-world trace-driven simulations.
We also show that, compared to existing baseline scheduling schemes, our GADGET algorithm can effectively meet the topology constraints, while achieving a good overall performance. 
%Interestingly, we show that even no resource violation is allowed in the rounding phase to obtain the integer solutions, a much better performance can still be achieved.
\end{list}

Collectively, our results contribute to a comprehensive and fundamental understanding of RAR-based machine learning system optimization.
The rest of this paper is organized as follows.
We review related work in Section~\ref{sec:Related}, and present preliminaries to familiarize readers with the necessary background of RAR in Section~\ref{sec:Preliminaries}.
We then present the system model, problem formulation, and an overview of our algorithmic ideas in Section~\ref{sec:model_formulation}.
We propose our online resource scheduling algorithm by decoupling it into time-independent subproblems in Section~\ref{sec:alg}, and then solve the NP-hard subproblem with our G-VNE approach in Section~\ref{sec:VNE}.
We evaluate performance of our proposed algorithms through numerical experiments in Section~\ref{sec:numerical}, and conclude this paper in Section~\ref{sec:conclusion}.


==> AllReduce_Scheduling_INFOCOM'21/Sec2-Related/Sec2-Related.tex <==
% !TEX root = ../AllReduce-Scheduling-INFOCOM'21.tex

\section{Related Work} \label{sec:Related}
Due to the rise of deep learning and their intensive computation workload, scheduling optimization for DDL to expedite the training process has attracted increasing attention recently.
To date, the PS-worker architecture~\cite{Li14:parameter-server} has been widely adopted and its scheduling design has been relatively well studied (e.g., \cite{Chilimbi14:Adam,Yan15:MLFramework_KDD, Sun17:Dorm, Bao18:OASiS}).
However, as pointed out in Section~\ref{sec:intro}, the PS-worker architecture suffers from communication bottlenecks and reliability limitations.
Thanks to its better scalability compared to the PS-worker architecture~\cite{Sergeev18:Horovod}, the RAR architecture has received strong interest in the research community and has been recently adopted by modern DDL frameworks.
% (e.g., TensorFlow~\cite{Abadi16:TensorFlow}, Pytorch~\cite{Paszke19:Pytorch}).
%These frameworks support overlapping communication with gradient computation, and many existing works focus on to achieve a better overlap.
So far, however, results on scheduling designs for the RAR architecture remain scarce.
To our knowledge, PACE~\cite{Bao20:all-reduce} is the only existing work in the literature designed for all-reduce tensors 
%(i.e., gradients to be transmitted) 
based on the RAR architecture, aiming at maximizing the overlap between communication and computation using DAG (directed acyclic graph) of DNN training.
However, the goal of PACE is to speed up the training process of a {\em single job}, instead of optimizing the scheduling of multiple jobs to improve the system-wide performance (e.g., minimize the average completion time).
In contrast, our goal in this work is to design the {\em first} scheduler tailored for the RAR-based DDL jobs in computing clusters.
We propose a theoretical framework that enables rigorous RAR-based DDL training resource optimization in large-scale %networked 
computing clusters (typically with a multi-layer hierarchical topology, e.g., fat-tree).



We note that there also exists other lines of research on resource scheduling for optimizing DDL training performance (e.g., latency, energy efficiency), but they are agnostic to the underlying distributed/parallel architectures.
Here, we also provide a quick overview, although they are not directly comparable to our work.
%\textcolor{red}{Many existing CPU/GPU schedulers~\cite{Xiao18:Gandiva,Gu19:Tiresias,Mahajan20:Themis} allow users to share resources in the computing cluster and run their jobs concurrently.}
%Many existing CPU/GPU schedulers~\cite{Xiao18:Gandiva,Gu19:Tiresias,Mahajan20:Themis} allow users to share resources in the computing cluster and run their jobs concurrently.
%Due to the rise of deep learning (DL) applications and their high computational workload, DDL training job scheduling systems have attracted a great amount of interest in recent years.
%These works aim to schedule DDL jobs and manage resources efficiently for a high-performance CPU/GPU-based clusters.
In~\cite{Gu19:Tiresias}, a GPU scheduler called Tiresias is proposed based on the assumption that DDL job performance could be estimated from historical job duration information.
%Studies~\cite{Jalaparti15:Network-aware,Tumanov16:Tetrisched} do not take the unique characteristics of DDL (e.g., iterativeness and convergence property) into consideration when the schedulers are designed.
%Some recent works~\cite{Zheng19:Cynthia,Liu19:Scheduling} focus on resource provisioning for multiple DDL jobs in the cloud.
%~\cite{Zheng19:Cynthia,Liu19:Scheduling} 
Meanwhile, a resource provisioning method called Cynthia was developed in~\cite{Zheng19:Cynthia} to study the impact of system heterogeneity, i.e., servers in the system may have different hardware configuration (e.g., CPU, amounts of memory), on both synchronous and asynchronous training, and to optimize the training performance.
%\textcolor{purple}{Wu: not clear what system heterogeneity in the DDL model means} 
Also, due to the growing training workloads that incur huge energy consumption in the GPU clusters, the design of energy-efficient scheduling algorithms also receives significant interest recently. 
For example, in~\cite{Mei17:energy,Chau17:energy}, various scheduling schemes are proposed for CPU/GPU hybrid clusters, aiming at maximizing the energy efficiency without significantly sacrificing the system performance.
We note, however, that all of these DDL scheduling algorithms are heuristic methods that do not provide performance guarantees.












==> AllReduce_Scheduling_INFOCOM'21/Sec3-Preliminaries/Sec3-Preliminaries.tex <==
% !TEX root = ../AllReduce-Scheduling-INFOCOM'21.tex

\begin{figure}[t!]
\includegraphics[width=.5\textwidth]{Figures/fig_rar_color-eps-converted-to.pdf}
\vspace{-.1in}
\caption{A three-worker illustrative example of the ring-all-reduce (RAR) process.}
\label{fig:ringallreduce}
\vspace{-.2in}
\end{figure}


\section{Distributed Learning with Ring-All-Reduce: A Primer}\label{sec:Preliminaries}

In this section, we  provide an overview on DDL training based on the RAR parallel computing architecture, to familiarize readers with necessary background and fix terminologies that will be used in this paper.

{\bf 1) Distributed Stochastic Gradient Descent (SGD):}
At the heart of deep learning lies an optimization problem in the form of $\min_{\w \in\mathbb{R}^d} \bar{L}(\w) \triangleq \frac{1}{N} \sum_{i=1}^{N} L(\w,\xi_i)$, where $\w$ contains the model parameters to be learned, $L(\w,\xi_i)$ is a loss function, 
%that evaluates the discrepancy between the output of a learning model (e.g., a deep neural network) and the ground truth of sample $\xi_i$, 
and $N$ is the total number of samples.
In an $w$-worker DDL system, the dataset is often partitioned and trained by each worker.
Let $\mathcal{D}_j$ denote the $j$-th partition of the dataset trained by a worker $j\in \{1,\ldots,w\}$.
Then, the training problem can be decomposed as $\min_{\w \in\mathbb{R}^d} \bar{L}(\w) = \sum_{j=1}^{w} \frac{|\mathcal{D}_j|}{N} L_j(\w)$, where $L_j(\w) \triangleq \frac{1}{|\mathcal{D}_j|} \sum_{i \in \mathcal{D}_{j}} L(\w,\xi_i)$.
To date, most DDL systems in practice adopt the distributed stochastic gradient descent (SGD) method, where, in iteration $k$, the weight parameter vector $\w$ is updated as 
$\w_{k+1} = \w_{k} - \eta_k \big( \sum_{j=1}^{n} \frac{|\mathcal{D}_j|}{N} \g_j^k \big)$, $k=1,2,\ldots$. 
Here $\eta_k$ is the step-size (aka learning rate) in iteration $k$, and $\g_j^k$ denotes the stochastic gradient computed by worker $j$ in iteration $k$.
%Also, the gradient computation at each worker is based on the celebrated {\em ``back-propagation''} scheme~\cite{Rumelhart86:BP}. % in deep learning training.

\smallskip
{\bf 2) The Ring-All-Reduce (RAR) Architecture:}
%Note that 
The above SGD update requires a weighted sum of all stochastic gradients, $\g_j$, $\forall j \in \{1,\ldots,w\}$ (the iteration index $k$ is omitted for notational simplicity).
To compute this weighted sum in the PS-worker architecture, each worker $j$ simply sends $\g_j$ to the PSs, which then perform the summation and return the result to each worker.
However, this implies that a $2wd$ amount of data exchange per iteration is required under the PS-worker architecture, which scales {\em linearly} as the number of workers increases and is problematic in large-scale DDL training.

To address this limitation, the more sophisticated RAR architecture is proposed.
The basic idea of RAR is to form a {\em ring} between the workers, where each worker performs gradient reduction (e.g., summation) and sharing by receiving gradients from its upstream worker and sending the local reduction result to its downstream worker.
In general, for a $w$-worker RAR structure, each worker splits its gradients into $w$ sub-vectors (see Fig.~\ref{fig:ringallreduce} for an example for $w=3$).
The RAR process is divided into two phases.
The first is the {\em ``Share-Reduce''} phase $(t=1,\ldots,w-1)$, where each worker sends its reduced sub-vector (i.e., the sub-vector sum) to its downstream worker, while receiving the reduced sub-vector from its upstream worker to compute a new reduced sub-vector.
The second phase is the {\em ``Share-Only''} phase  $(t=$ $w,\ldots,2w-2)$, where each node sends its newly received fully-reduced sub-vector to its downstream worker, while receiving a new fully-reduced sub-vector from its upstream worker.
Since each worker sends $\frac{d}{w}$ amount of data for $2(w-1)$ times, the total amount of data each worker sends is $\frac{2d(w-1)}{w}$, which is asymptotically {\em independent} of $w$ as $w$ gets large. %(also referred to as being {\em bandwidth-optimal} in the literature).


\smallskip
{\bf 3) Per-Iteration Training Time for RAR-Based DDL:}
%With the above basics of RAR, we are now in a position to characterize the per-iteration training time of RAR.
Consider a $w$-worker RAR-based DDL training job.
We use $b$ to denote the bandwidth between workers.
%We use $B_j$ to denote the bandwidth between workers of job $j$.
% (e.g., sum of floating points when using GPU).
%Assume that the workers have same performance and specification, and we focus on synchronous training.
We use $G$ to denote the computation speed of a worker.
Since each worker sends a gradient sub-vector of size $d/w$ at each time step for $2(w-1)$ times, the transmission time can be computed as $\frac{2d(w-1)}{wb}$.
Also, since it takes $w-1$ times in total to perform gradient sub-vector summations, the computation time can be computed as $\frac{d(w-1)}{wG}$.
%Recall that all workers need to be synchronized before they proceed to the next iteration since we focus on the synchronized training.
%In other words, the slowest link between all workers will become the bottleneck, and we let $B_j\triangleq\min_{(\omega_1,\omega_2)\in\mathcal{W}_j}B_j^{\{\omega_1,\omega_2\}}$, where $\mathcal{W}_j$ is the set of links between workers of job $j$.
Hence, the total time for a single RAR operation is $\frac{d(w-1)}{w} [\frac{2}{b}+\frac{1}{G} ]$.
In each iteration of RAR-based DDL training, in addition to the all-reduce operation time, each worker needs to perform a forward pass (FP) and a backward pass (BP) to compute the stochastic gradients.
% We let $t_f$, $t_b$ denote the FP and BP time, respectively.
The FP time can be computed as $t^{f}M$, where $t^f$ is the model-dependent per-sample FP time and $M$ is mini-batch size.
% \begin{align}
%  t_f=\lambda_f B,  
% \end{align}
%The BP time $t^b$ is independent of the mini-batch size and is model-dependent.
The BP time $t^b$ is independent of the mini-batch size.
% \begin{align}
%   t_b=\lambda_b.  
% \end{align}
% where $\lambda_f$ and $\lambda_b$ are DNN-model dependent workload coefficients.
% In practice, for a given model, we can measure $\lambda_f$ and $\lambda_b$, which will remain unchanged throughout the entire training process.
In addition, there is extra latency $\gamma$ caused by communication overhead (e.g., ACK time for message transmission, negotiation time among all workers before conducting RAR~\cite{Sergeev18:Horovod}). 
By putting all the above time consumption components together, we have the per-iteration training time $\tau$ for RAR-based DDL as:
% \begin{align}
%     \label{totaltime} a+t_fB+t_b
% \end{align}
% Hence we can have the time to complete All-Reduce on job $i$:
\begin{align} \label{per-iteration-time}
\tau = \frac{d(w-1)}{w} \bigg[\frac{2}{b}+\frac{1}{G} \bigg]+t^fM+t^b + \gamma. \footnotemark
\end{align}
\footnotetext{In this paper, we focus on GPU computation and network communication times and neglect the data IO latency due to the use of high-speed solid state drives (SSDs), short pre-fetch time of pre-stored training programs, and overlapping of data chunks fetching and training through pipelining.}
We can see that $\tau$ depends on the learning model size, worker communication and computation speeds, batch size, communication overhead, and FP/BP times (in turn, the learning model), but is asymptotically upper bounded by $d(\frac{2}{b}+\frac{1}{G}) +t^fM+t^b + \gamma$ as the number of workers $w$ goes to infinity.





==> AllReduce_Scheduling_INFOCOM'21/Sec4-Model/Sec4-Model.tex <==
% !TEX root = ../AllReduce-Scheduling-INFOCOM'21.tex


\section{System Model and Problem Formulation} \label{sec:model_formulation}\label{sec:general_framework}

%In this section, we first characterize per-iteration execution time using ring All-reduce collective operation, followed by introducing our system model.
%Then we present our general problem formulation for DDL training in shared, multi-tenant GPU clusters.
%Finally, we provide the overview of our proposed online resource scheduling algorithm design.
%
In this section, we will present a general analytical framework for resource scheduling and allocation for RAR-based DDL training performance optimization.
%Then, we will provide several applications of our analytical framework in Section~\ref{subsec:applications}.
%, then present our general problem formulation.
%
%\subsection{Analytical Framework for RAR-Based DDL Optimization} \label{subsec:general_framework}
%\textcolor{purple}{Wu: this subsection title may be removed since there is only one subsection}

%Consider scheduling RAR-based DDL training jobs in 

Consider a %networked 
computing cluster with a set of physical servers denoted as $\mathcal{S}$.
Each server has a certain amount of computing resources (e.g., GPUs, memory).
The system is time-slotted with horizon $\mathcal{T} \triangleq \{1, 2, \cdots, T\}$.
%For each $t \in \mathcal{T}$, an RAR-based DDL job randomly arrives and competes the shared resources with unfinished jobs.
Over time, RAR-based DDL jobs dynamically arrive and compete for the shared resources with unfinished jobs.
Let $a_{i}$ denote the arrival time of job $i$, which is {\em unpredictable} to the scheduler.
Let $\mathcal{I}$ denote the set of jobs arrived over time horizon $\mathcal{T}$.
The jobs are {\em preemptive} if resources are insufficient and could be resumed later.\footnote{Flexible resource allocation enabled by containers can be exploited to suspend a job and reclaim its resources without losing the execution progress~\cite{Chen17:USENIX}.}
All jobs' workers are implemented as containers. 
Next, we will develop RAR-based DDL scheduling models in detail.

\smallskip
{\bf 1) Resource Constraint Modeling:} 
% We use a binary variable $x_j$ to indicate whether job $j$ is executed ($x_j=1$) or not ($x_j=0$).
%The first component is resource constraints modeling.
We let $y_{is}[t]$ denote the number of workers scheduled on server $s$ for job $i$ in time-slot $t$.
%Let $N_i$ denote the number of data chunks of job $i$.
%Let $N_i$ denote the largest number of workers allocated to job $i$.
%%Since the number of assigned concurrent workers in each time-slot should be no more than the total data chunks of job $i$ (denoted by $N_i$), we have:
%For example, if it is the number of data chunks for job $i$, then this constraint ensure that no workers will be idle since each data chunk is processed by at most one worker in each time slot.
%and each data chunk is processed by at most one worker in each time slot such that data chunks are trained evenly over time.
Let $N_i$ be the largest number of assigned concurrent workers in each time-slot, we have: 
%(jobs using beyond a certain amount of GPUs may experience reliability failures more often~\cite{Jeon2018:multi-tenant}), we have:
%Let $N_i$ be the maximum number of iterations to be trained of job $i$, which is determined by the user upon job $i$'s submission, we have:
%To model that the largest number of assigned concurrent workers is no more than the number of data chunks $N_i$ (otherwise some workers will be idle),  we have:
\begin{align}
 \label{ctr:maxworker}\sum_{s\in\mathcal{S}}y_{is}[t]\leq N_i, \quad\forall i\in\mathcal{I},  \forall t \in \mathcal{T}. 
\end{align}

Let $\mathcal{R}$ denote the set of computing resources (e.g., GPUs, memory, training time budget).
Let $l_i^r$ be the amount of type-$r$ resource consumed by each worker of job $i$.
We use $F_i^r$ to denote the maximum type-$r$ resource demand requested by job $i$.
To ensure that job $i$ does not exceed type-$r$ resource's limit, we have:
\begin{align}
    \label{ctr:iter}&\sum_{t\in\mathcal{T}}l_i^r \sum_{s\in\mathcal{S}}y_{is}[t]\leq F_i^r,\quad\forall i\in\mathcal{I}, \forall r \in \mathcal{R}.
\end{align}
%Also, let $O_i$ be the maximum number of iterations to be trained of job $i$, which is specified upon its submission. We have:
%\begin{align}
%    \label{ctr:maxiter}&\sum_{t\in\mathcal{T}}\sum_{i\in\mathcal{I}} y_{is}[t]\leq O_i \quad\forall i\in\mathcal{I}.
%\end{align}

Let $C_s^r$ denote the type-$r$ resource capacity of server $s$.
To ensure that server's type-$r$ limit is not violated, we have:
\begin{align}
    \label{ctr:cap}&\sum_{i\in\mathcal{I}} l_i^r y_{is}[t]\leq C_s^r, \quad\forall s\in\mathcal{S}, t\in\mathcal{T}, \forall r \in \mathcal{R}.
\end{align}

%To ensure that no workers can be placed on server $s$ for job $i$  if job $i$ does not use server $s$ in time-slot $t$, we have:
%\begin{align}
%\label{ctr:placement}(1-x_{is}[t])y_{is}[t]=0, \quad\forall i\in\mathcal{I},s\in\mathcal{S},t\in\mathcal{T}.
%\end{align}
%We can see from the above that $x_{is}[t]=0$ will force $y_{is}[t]=0$.
We use a binary variable $x_{is}[t]=1$ to indicate that job $i$ uses server $s$ in each time-slot $t$ and let $x_{is}[t]=0$ if otherwise.
Note that, when server $s$ is used for job $i$, $y_{is}[t]$ should not exceed any maximum resource demand $F_i^r$,  the resource capacity of server $s$, and the largest number of workers of job $i$ in each time-slot $t$.
%i.e., $y_{is}[t]\leq\min\{N_i, C_s^r/l_i^r, F_i^r/l_i^r,\forall r \}$.
%Note that, when server $s$ is used for job $i$, $y_{is}[t]$ should exceed neither any resource limit $C_s^r$ nor the number of data chunks of job $j$ in each time-slot $t$, i.e., $y_{is}[t]=\min\{N_i, C_s^r/l_i^r, \forall r \}$.
Also, observe that $x_{is}[t]=0$ forces $y_{is}[t]=0$. 
Combining these facts yields:
\begin{align}
\label{ctr:placement-r}y_{is}[t]\!\leq\!x_{is}[t]\min \bigg\{N_i,\frac{C_s^r}{l_i^r}, \frac{F_i^r}{l_i^r}, \forall r \bigg\}, \forall i\!\in\!\mathcal{I},s\!\in\!\mathcal{S},t\!\in\!\mathcal{T}. \!\!\!
\end{align}
To ensure no workers are allocated before jobs arrive, we have:
\begin{align}
    &y_{is}[t]=0, \quad \forall i\in\mathcal{I}, s\in\mathcal{S}, t<a_i.
\end{align}

\smallskip
{\bf 2) RAR Topological Constraint Modeling:} 
A key component in scheduling an RAR-based DDL training job is to guarantee that the {\em physical network topology} corresponding to the resource scheduling decisions should be {\em compatible} with the {\em logical topology} of the job's computational graph.
Toward this end, we note that the computational graph of an RAR-based DDL training job $i$ is a {\em directed ring graph} $G_i=(V_i, E_i)$, where $V_i$ is the set of logical vertices representing workers, and $E_i$ represents the set of logical edges denoting the RAR directions between the workers.
Also, physical servers and network links in the cluster can be modeled as a directed substrate graph. %\textcolor{purple}{Wu: what is a substrate graph?} $G_s=(V_s, E_s)$, where $V_s$ is the set of physical servers and $E_s$ is the set of network links that connect the servers. 
%For example, a typical substrate graph topology in computing clusters is the so-called ``fat tree.''
%This problem can be translated into virtual network embedding problem (VNEP) with the goal to jointly map virtual nodes to physical servers and map virtual edges onto paths in the substrate graph.
Next, we model the topological constraints.

%We let a binary variable $x_{is}[t]=1$ to indicate job $i$ uses server $s$ in time-slot $t$ and $x_{is}[t]=0$ to indicate otherwise.
We use $\mathcal{P}_{ss'}[t]$ to denote the set of all possible paths between severs $s$ and $s'$ in the physical substrate graph in time-slot $t$.
We use a binary variable $r_{ss'}^{(p,i)}[t]=1$ to indicate that a path $p\in \mathcal{P}_{ss'}[t]$ is used by job $i$ in time-slot $t$, and let $r_{ss'}^{(p,i)}[t]=0$, otherwise.
If neither server $s$ nor $s'$ hosts any worker of job $i$ in time-slot $t$, then $r_{ss'}^{(p,i)}[t]=0$, which implies:
%%Note that  $r_{ss'}^{(i)}[t]=1$ indicates inter-connect communication is conducted for job $i$ in time slot $t$.
\begin{align}
\label{ctr:link}r_{ss'}^{(p,i)}[t]\leq x_{is}[t]x_{is'}[t], \forall s,s'\!\in\!\mathcal{S}, p\!\in\!\mathcal{P}_{ss'}[t], i\!\in\!\mathcal{I}, t\!\in\!\mathcal{T}.
%\label{ctr:link}r_{ss'}^{(i)}[t]=\mathds{1}\{\}, \forall s,s'\in\mathcal{S}, i\in\mathcal{I}, t\in\mathcal{T}.
%\label{ctr:link}r_{ss'}^{(i)}[t]\geq\prod_{\tilde{s}\in p} x_{i\tilde{s}}[t], \forall  p\in\mathcal{P}^{(i)}_{ss'}[t], s,s'\in\mathcal{S}, i\in\mathcal{I}, t\in\mathcal{T}.
\end{align}
Also, we use $b_i$ and $B_{\min}^p[t]$ to denote the reserved bandwidth requirement of job $i$ and the bottleneck link capacity of path $p \in \mathcal{P}_{ss'}[t]$, respectively.
To ensure that the bottleneck link capacity in any activated path $p$ is not exceeded, we have:
%should ensure that the bottleneck link's bandwidth capacity will not be violated.
%Thus, we have:
\begin{align}
\label{ctr:inter}&\sum_{i\in\mathcal{I}}r_{ss'}^{(p,i)}[t]b_i \leq B^p_{\min}[t], \forall s,s'\in\mathcal{S}, p\in \mathcal{P}_{ss'}[t], t\in\mathcal{T}.
\end{align}

  \begin{figure}[t!]
  \includegraphics[width=.52\textwidth]{Figures/fig_topology-eps-converted-to.pdf}
  \caption{Various placement schemes with three workers.}
  \label{fig:placement}
  \vspace{-.2in}
\end{figure}


%We use $\mathcal{S}_i[t]$ be the set of servers that are used by job $i$ at time $t$.
Next, to ensure that the allocated workers of job $i$ can indeed form a directed ring graph, we consider two cases.
First, if only one server hosts all workers for job $i$, then the cyclic constraint is automatically satisfied since a server can support any computational graph topology for co-located workers (Fig.~\ref{fig:placement}(a)).{\footnote{Servers in Fig.~\ref{fig:placement} are connected cyclically, i.e., there are communication links between servers 1 and 2, 2 and 4, 4 and 3, 3 and 1.}
Second, if workers are located on different servers, it can be observed that each server that hosts some of job $i$'s workers (i.e.,  $x_{is}[t]=1$) should have a degree of {\em exactly two} for job $i$'s paths in order to form a cycle (Fig.~\ref{fig:placement}(b)-(c)).
These two cases can be compactly written in one constraint as:
\begin{align} 
&\mathds{1}\bigg\{\sum_{s'\in\mathcal{S}}x_{is'}[t] \!-\!1\!>\!0 \bigg\} \bigg(\sum_{s' \in \mathcal{S}_i[t]} \sum_{p\in\mathcal{P}_{ss'}[t]}r_{ss'}^{(p,i)}[t]\!-\!2\bigg) = 0, \nonumber\\
  \label{ctr:cycle}&\hspace{1.5in} \quad\forall i\in\mathcal{I}, s\in\mathcal{S}, t\in\mathcal{T}.
\end{align}
where $\mathcal{S}_i[t]$ denotes the set of servers containing job $i$ at time $t$.
To see why Eq.~(\ref{ctr:cycle}) is a valid constraint, note that if all workers of job $i$ are hosted by server $s$, we have $\mathds{1} \{\sum_{s'\in\mathcal{S}}x_{is'}[t] - 1 > 0\} = 0$, which implies Eq.~\eqref{ctr:cycle} trivially holds.
%Otherwise, the term $(\sum_{s' \in \mathcal{S}_i[t]} \sum_{p\in\mathcal{P}_{ss'}[t]}r_{ss'}^{(p,i)}[t]-2) = 0$ enforces the degree of two at server $s\in\mathcal{S}_i[t]$. 
Note also that the first summation in this term is over the set $\mathcal{S}_i[t]$.
This guarantees that there is only one big cycle instead of multiple small cycles.


\smallskip
{\bf 3) Objective Function and Problem Statement: } 
Let $\mu_{i}(\cdot)$ be the utility function associated with job $i$'s resource allocation, which is {\em non-decreasing} and concave to represent the ``diminishing return effect.''
%We use the function  $\mu_i(\sum_t p_i \sum_{s\in\mathcal{S}}y_{is}[t])$ to denote the utility function of job $i$.
%which can deliver the results with respect to partial training iterations $\sum_tl_i\sum_{s\in\mathcal{S}}y_{is}[t]$.
In this paper, our goal is to maximize the overall utility of all jobs.
Let $\zeta_i$ represent some general notion of ``per-worker efficiency/cost'' (see three concrete examples next). 
Putting all modeling together, the DDL job scheduling problem (DDLJS) can be formulated as:
\begin{align*}
{\bf DDLJS: } \underset{\mathbf{x,y}}{\text{Maximize }} &\sum_{i\in\mathcal{I}}\mu_i \Big( \zeta_i \!\! \sum_{t\in\mathcal{T}} \sum_{s\in\mathcal{S}}y_{is}[t] \Big)\\
    \text{subject to } 
    &\text{Constraints }  (\ref{ctr:maxworker})-(\ref{ctr:cycle}).  
\end{align*}

%Clearly, Problem~DDLJS is an online (i.e., the scheduler does not have the knowledge of arrival times $\{a_i, \forall i\}$) and mixed integer non-linear programming (MINLP) problem, which is NP-Hard in general.

%Before developing algorithms to solve the problem, we provide several applications of our general analytical framework to further motivate and highlight its relevance in practice.
We note that Problem~DDLJS is a general analytical framework that has many applications.
Here, we provide three examples to highlight its practical relevance:
{\bf 1) Excessive Training Avoidance~\cite{Jeon2018:multi-tenant}:} 
Here, $\zeta_i$ can represent the number of training iterations per-unit time of each worker of job $i$, which can be obtained by inverting Eq.~(\ref{per-iteration-time}).
The utility function can be chosen as $\mu(k) = (O(1/\sqrt{k}))^{-1} = C\sqrt{k}$ for some $C>0$, which is the typical convergence rate of SGD-type algorithms with respect to the iteration index $k$.
{\bf 2) Energy-Efficiency Optimization~\cite{Chau17:energy}:} 
Here, $\zeta_i$ denotes the per-worker power consumption of job $i$.
We can choose $\mu(\cdot) = -c(\zeta_i \sum_{t\in\mathcal{T}} \sum_{s\in\mathcal{S}}y_{is}[t])$, where $c(\cdot)$ is a quadratic function, which is often used in the power system literature to model energy consumption costs.
{\bf 3) Resource Fairness in Training:} Here, we can let $\zeta_i = 1$, $\forall i$, and adopt the classical ``proportional fairness'' utility function~\cite{Hou14:Proportional-Fair}, i.e., $\mu(\cdot) = \log(\cdot)$.




















==> AllReduce_Scheduling_INFOCOM'21/Sec5-Algorithm/Sec5-Algorithm.tex <==
% !TEX root = ../AllReduce-Scheduling-INFOCOM'21.tex

\section{Solution Approach} \label{sec:alg}

%In this section, we focus on developing algorithms to solve Problem~DDLJS.
Problem~DDLJS is a challenging {\em online} optimization problem (the scheduler does not have arrival information $\{a_i, \forall i\}$).
%, where some performance loss is inevitable due to uncertainty in future information.
What exacerbates the problem is the fact that even its offline planning version (assuming $\{a_i, \forall i\}$ are known beforehand) is a mixed-integer non-convex programming (MINCP) problem, which is NP-Hard in general.
%Too see this, note that Eq.~(\ref{ctr:cycle}) involves the product of $x$- and $r$- variables, which leads to integer bilinear constraints.
Moreover, Eq.~(\ref{ctr:cycle}) contains an indicator function that is not amenable to conventional optimization techniques.
In light of all these challenges, our goal in this paper is to pursue an online approximation algorithmic design that offers theoretical competitive ratio guarantee.


\subsection{Basic Idea}

%In order to effectively solve Problem~DDLJS, we design a novel approximation algorithm that leverages submodularity with partition matroid, and VNE techniques, to deal with the aforementioned challenges.
To overcome the above challenges, we propose an online algorithmic design called GADGET (\underline{g}reedy ring-\underline{a}ll-reduce \underline{d}istributed \underline{g}raph \underline{e}mbedding \underline{t}echnique).
%, which enjoys a provable competitive ratio guarantee.
Our basic idea of GADGET contains two key steps:
i) Through a careful examination, we show that Problem~DDLJS is submodular with respect to scheduling decisions in the {\em temporal} domain.
Thus, it is possible to design a temporally greedy scheduling algorithm with a provable competitive ratio;
ii) For the resource allocation subproblem in each time-slot that remains NP-Hard, we show that it can be viewed as a {\em generalized} virtual network embedding problem (G-VNE).
As a result, it is also possible to (non-trivially) modify existing VNE techniques (see, e.g,. \cite{Rost18:VNE} and references therein) to adapt to our setting and solve each subproblem with provable approximation ratio guarantee.
We illustrate the basic idea of our GADGET algorithm in Fig.~\ref{fig:idea}.
In what follows, we will discuss these two key steps in detail.
\begin{figure}[t!]
  \includegraphics[width=1\columnwidth]{Figures/fig_idea_overveiw-eps-converted-to.pdf}
%   \vspace{.08in}
  \caption{Algorithmic idea overview.}
  \label{fig:idea}
  \vspace{-.2in}
\end{figure}


% The offline maximization problem~DDLJS is an MINLP.
% It is highly non-trival to solve such an MINLP even with the complete knowledge in the entire time span $\mathcal{T}$.

\vspace{-.1in}
\subsection{An Online Temporally Greedy Approach}\label{subsec:greedy}
In this subsection, we establish the submodularity of Problem~DDLJS over the temporal domain.
First, consider the following online {\em temporally greedy} algorithm.
We let $z_{i,t}\triangleq\sum_{\tau=1}^t \sum_{s\in\mathcal{S}}y_{is}[\tau]$ be the {\em accumulative} number of worker-time allocated for job $i$ up to time $t$.
Define $\mathcal{I}[t]\triangleq\{i \in \mathcal{I}: t\geq a_i\text{ and } z_{i,t-1} < \min_{r\in\mathcal{R}} F_i^r/l_{i}^{r} \}$ as the set of jobs that are {\it active} (i.e., in-training and not resource-violated in time-slot $t$). 
Given the scheduling $\{z_{i,t-1}\}_{i\in\mathcal{I}[t]}$ in previous time slots, we greedily find the resource allocation in time-slot $t$ by solving the following optimization problem:
\begin{align}
\label{problem:pt}\text{ Maximize }
      &\sum_{i\in\mathcal{I}[t]}\mu_i \Big( \zeta_i\sum_{s\in\mathcal{S}}y_{is}[t]+\zeta_iz_{i,t-1} \Big)\\
    \text{subject to } 
    &\label{ctr:iter_t} \sum_{s\in\mathcal{S}}y_{is}[t]\leq \Big(\min_{r\in\mathcal{R}} \frac{F_i^r}{l_{i}^{r}} \Big)\!-\!z_{i,t-1}, \,\forall i\!\in\!\mathcal{I}[t],\\
    &\nonumber\text{Constraints }(\ref{ctr:maxworker}), (\ref{ctr:cap})-(\ref{ctr:cycle}) \text{ only at $t$ }, \forall i\!\in\!\mathcal{I}[t], \\ %\text{w/o } \forall t\!\in\!\mathcal{T},\\
    &\nonumber y_{is}[t] \in \mathbb{Z}_{+}, \,\, x_{is}[t]\!\in\!\{0,1\},\forall i\!\in\!\mathcal{I}[t], s\in\mathcal{S}\nonumber.
\end{align}
Constraint~(\ref{ctr:iter_t}) ensures that the accumulated ``worker-time product'' in time slot $t$ does not exceed the remaining worker-time-product limit (determined by the bottleneck resource type) for all active jobs.
%Constraints~(\ref{ctr:Mc1_t})-(\ref{ctr:Mc3_t}) are logically equivalent McCormick inequalities of Constraint~(\ref{ctr:link}).
%Similarly, Constraint~(\ref{ctr:Mc4_t})-(\ref{ctr:cycle_t}) are logically equivalent inequalities of Constraint~(\ref{ctr:cycle}), where we let $w_{ss'}^{(i)}[t]=r_{ss'}^{(i)}[t]x_{is}[t]$.
%Note that $r_{ss'}^{(i)}[t], w_{ss'}^{(i)}[t]\in\{0,1\}$.
Note that Problem~(\ref{problem:pt}) remains a challenging NP-Hard packing problem, for which an approximation algorithm will be developed later in Section~\ref{sec:VNE}.
%%%%%approximation algorithm%%%%%%
With Problem~(\ref{problem:pt}), our online temporally greedy algorithm is presented in Algorithm~\ref{alg:fractional_scheduling}.
%, where in each time slot, it greedily finds the local scheduling with performance bound (see Section~\ref{sec:VNE}) without knowing the future arrivals.

\begin{algorithm}
\SetAlgoLined
% \KwResult{The $\epsilon$-approximation fractional solution for each job $i$. }
\label{line:intialization}\textbf{Initialization:} Set $z_{i,t}\leftarrow0,\forall t\in\mathcal{T}, i\in\mathcal{I}$\;
 \label{line:iterate}\For{$t\in\mathcal{T}$}{
  \label{line:J[t]} $\mathcal{I}[t]\!\triangleq\!\{i\in\mathcal{I}: t\geq a_i\text{ and }z_{i}[t\!-\!1] \!\!< \!\min_{r\in\mathcal{R}} F_i^r/l_i^r \}$\;
  \label{line:subproblem1}$y_{is}[t]\leftarrow$ Solutions of Problem~(\ref{problem:pt}) using Algorithm~\ref{alg:round} developed in Section~\ref{sec:VNE}\;
%   \label{line:rounding} Round $y_i[t]$ to $\hat{y}_i[t]$ using Algorithm~(\ref{alg:round})(to be specified)\;
  \Return $y_{is}[t]$\;
  \label{line:update_z}$z_{i,t} \leftarrow z_{i,t-1} + \sum_{s\in\mathcal{S}}y_{is}[t]$\;
  }
 \caption{Online Temporally Greedy Approach.}
 \label{alg:fractional_scheduling}
\end{algorithm}


Next, we show that Algorithm~\ref{alg:fractional_scheduling} provides competitive ratio guarantee by proving that Problem~DDLJS is submodular over the temporal domain.
For the paper to be self-contained, we restate some necessary basics of submodular optimization and matroid theory here, and refer readers to standard sources of submodular optimization (e.g.,~\cite{Schrijver03:combinatorial}) for further details.

\begin{defn}[Submodularity]
\label{def:3}A set function $f(\cdot): 2^\mathcal{V}\rightarrow\mathds{R}$ is submodular if for every $\mathcal{B}\subseteq\mathcal{V}$, and $\mathcal{A}'\subseteq\mathcal{A}\subseteq\mathcal{V}$, we have $f(\mathcal{A}\cup\mathcal{B}) - f(\mathcal{A})\leq f(\mathcal{A}'\cup\mathcal{B}) - f(\mathcal{A}')$.
%\begin{align*}
%f(\mathcal{A}\cup\mathcal{B}) - f(\mathcal{A})\leq f(\mathcal{A}'\cup\mathcal{B}) - f(\mathcal{A}').
%\end{align*}
\end{defn}
An important subclass of submodular functions are those that have the monotone property defined as follows:
\begin{defn}[Monotonicity]
A set function $f(\cdot): 2^\mathcal{V}\rightarrow\mathds{R}$ is monotone if for every $\mathcal{A}\subseteq\mathcal{B}\subseteq\mathcal{V}$, we have $f(\mathcal{A})\leq f(\mathcal{B})$.
\end{defn}
%Note that a set function $f$ is monotone if and only if all its discrete derivatives are nonnegative.
%That is, $\delta_f(v | \mathcal{A})\geq 0$, for every $\mathcal{A}\subseteq \mathcal{V}, v\in\mathcal{V}$.
In this paper, we focus on non-negative monotone submodular functions.
Submodular optimization is also closely related to the notion of matroid, which is defined as follows:
\begin{defn}[Matroid]
A matroid is a pair $(\mathcal{V}, \mathcal{J})$ such that $\mathcal{V}$ is a finite set, and $\mathcal{J}\subseteq 2^\mathcal{V}$ is a collection of independent subsets  of $\mathcal{V}$ satisfying: 1) $\emptyset\in\mathcal{J}$; 2) for $\mathcal{A}\subseteq\mathcal{B}\subseteq\mathcal{V}$, if $\mathcal{B}\in\mathcal{J}$, then it implies $\mathcal{A}\in\mathcal{J}$; 3) if $\mathcal{A,B}\in\mathcal{J}$, and $|\mathcal{A}|<|\mathcal{B}|$, then $\exists \,\, v\in\mathcal{B}\setminus\mathcal{A}$ such that $\mathcal{A}\cup\{v\}\in\mathcal{J}$.
%\begin{align*}
%&\emptyset\in\mathcal{I}\\
%&\mathcal{A}\subseteq\mathcal{B}\subseteq\mathcal{V}, \text{if }\mathcal{B}\in\mathcal{I}, \text{then it implies }\mathcal{A}\in\mathcal{I}
%\end{align*}
\end{defn}
Matroids have many interesting properties and subclasses.
One important subclass of matroids that is useful in this paper is the partition matroid, which is defined as follows:
\begin{defn}[Partition Matroid]
%Let $\mathcal{V}_j$ be a collection of disjoint subsets of $\mathcal{V}$.
Partition $\mathcal{V}$ into disjoint subsets $\{\mathcal{V}_{j}\}$.
Let $0 \!\leq\! \nu_j \!\leq\! |\mathcal{V}_j|$, $\forall j$ be integers associated with the $\mathcal{V}_j$'s.
%If a set of elements $\mathcal{S}$ is independent, i.e., $\mathcal{S}\in\mathcal{V}$ if and only if $|\mathcal{S}\cap \mathcal{V}_i|\leq \nu_i, \forall i$, then the collection $\mathcal{I}$ of independent sets forms a partition matroid.
%Define a subset $\mathcal{H} \!\in\! \mathcal{J}$ to be independent if and only if $|\mathcal{H} \!\cap\! \mathcal{V}_j| \!\leq\! \nu_j, \forall j$.
%The sets satisfying this condition are partition matroids.
Define a collection of subsets $\mathcal{J} \!=\! \{ \mathcal{H} \!\in\! \mathcal{V}: |\mathcal{H} \!\cap\! \mathcal{V}_j| \!\leq\! \nu_j, \forall j\}$.
Then, the pair $(\mathcal{V}, \mathcal{J})$ is a partition matroid.
\end{defn}

We now show that Problem~DDLJS is a submodular optimization problem in the temporal domain.
To avoid ambiguity, we will use the term {\em ``schedule''} to refer to an $(\x,\y)$-decision over the entire time horizon $\mathcal{T}$;
and we use the term {\em ``allocation''} to refer to an $(\x,\y)$-decision in a particular time-slot (i.e., a ``snapshot'' in time).
We let $\mathcal{H} \triangleq \{ \mathcal{H}[t], t\in \mathcal{T} \}$ be the space of all  schedules, where $\mathcal{H}[t]$ denotes the space of all resource allocation in time-slot $t$ (which may or may not be feasible).
Define the ground set  $\mathcal{V} \triangleq \{y_{is}[t], \forall i,s,t | y_{is}[t]\in\mathcal{H}[t], \forall t \} \subset \mathbb{Z}_{+}^{|\mathcal{I}|\times |\mathcal{S}|\times|\mathcal{T}|}$ to be the space of all possible schedules of the $y$-components.
Also, let $\mathcal{V}[t] = \{y_{is}[t], \forall i, s | y_{is}[t]\in\mathcal{H}[t]\} \subset \mathbb{Z}_{+}^{|\mathcal{I}|\times |\mathcal{S}|}$ denote the feasible $y$-allocation space in time-slot $t$.
Clearly, $\{\mathcal{V}[t], t \in \mathcal{T}\}$ is a partition of $\mathcal{V}$ since $\mathcal{V}[t_1] \cap \mathcal{V}[t_2] = \emptyset$.
%, i.e., all possible schedules at time $t$.
Now, we choose $\nu_t = 1$, $\forall t \in \mathcal{T}$.
Consider any schedule $\mathcal{E} \in \mathcal{V}$. 
Since at most one resource allocation decision can be chosen in each time slot in $\mathcal{E}$, we have $|\mathcal{E} \cap \mathcal{V}[t]| \leq1 = \nu_t$, $\forall t$.
%we have $\mathcal{E}\subseteq \mathcal{V}$ is independent if and only if $|\mathcal{H}\cap \mathcal{V}[t]|\leq 1, \forall t$.
Let $\mathcal{J}$ be the collection of all such feasible schedules $\{\mathcal{E}\}$.
Then, the pair $(\mathcal{V},\mathcal{J})$ containing all schedules forms a partition matroid, and finding an optimal feasible schedule is equivalent to finding an optimal independent set of this partition matroid.


Next, we let $z_i[t] = \sum_{s\in\mathcal{S}}y_{is}[t]$ denote the total number of workers of job $i$ in time-slot $t$.
Clearly, $z_i[t]=0, \forall t < a_i$.
Recalling the definition of $z_{i,t}$, we have $z_{i,t}=z_i[a_i]+z_i[a_i + 1] + \cdots+z_i[t]$.
For any schedule $\mathcal{E}$ (could be infeasible), we define $z^{\mathcal{E}}_{i}[t] \triangleq \sum_{\{ y_{is}[t] \in \mathcal{E} \cap \mathcal{V}[t] \}} y_{is}[t] $.
Accordingly, we define $z_{i,t}^\mathcal{E} \triangleq z_i^\mathcal{E}[a_i]+\cdots+z_i^\mathcal{E}[t]$.
Then, we can rewrite the objective function in (\ref{problem:pt}) as $F(\mathcal{E}) \triangleq \sum_{i\in\mathcal{I}} \mu_{i}(\zeta_i z_{i,T}^{\mathcal{E}})$.
%Define a set function $F_{\mathcal{E}}(t)$ as: 
%$$
%F(\mathcal{E}) \triangleq \sum_{i\in\mathcal{I}} \mu_{i}(\zeta_i z_{i,T}^{\mathcal{E}}).
%$$
Since $\mu_{i}(\cdot)$ is concave and increasing, $F(\mathcal{E})$ is monotonically increasing as $t$ increases.
Next, we show that $F(\mathcal{E})$ is also submodular.
\begin{lem}
$F(\mathcal{E})$ is a submodular function.
\end{lem}

\begin{proof}
%To show that $F_{\mathcal{E}}(t)$ is a submodular function, 
We pick two schedules $\mathcal{A}$ and $\mathcal{B}$ such that $\mathcal{A}\subseteq\mathcal{B}\subseteq\mathcal{V}$.
Now, for a resource allocation decision $v \in \mathcal{V}[t]$ in time-slot $t$.
Consider the following two cases:
\begin{list}{\labelitemi}{\leftmargin=1em \itemindent=0.em \itemsep=.2em}
\item Case 1) $v\in\mathcal{B}$:
In this case, we have $F(\mathcal{A}\cup\{v\}) - F(\mathcal{A}) \geq F(\mathcal{B}\cup\{v\}) - F(\mathcal{B}) =0$, which holds trivially.

\item Case 2) $v\not\in\mathcal{B}$: In this case, we have
\begin{align*}
&\!\!\!\! F(\mathcal{B} \!\cup\! \{v\}) \!-\! F(\mathcal{B}) \!=\!\! \sum_{i\in\mathcal{I}}\big(\mu_i(\zeta_i z_{i,T}^\mathcal{B} \!+\! \zeta_iz_i^v[t]) \!-\! \mu_i(\zeta_iz_{i,T}^\mathcal{B})\big) \\
%
 &\!\!\!\!\!\! \overset{(a)}{\leq} \!\!\sum_{i\in\mathcal{I}} \big(\mu_i(\zeta_i z_{i,T}^\mathcal{A} \!+\! \zeta_i z_i^v[t]) \!-\! \mu_i(\zeta_i z_{i,T}^\mathcal{A}) \big) \!\!=\!\! F(\mathcal{A} \!\cup\! \{v\}) \!-\! F(\mathcal{A}),
\end{align*}
\end{list}
%thus $z_{i,T}^\mathcal{B}\geq z_{i,T}^\mathcal{A}$ since $\mathcal{A}\subseteq\mathcal{B}$.
where $(a)$ follows from $\mu_i(\cdot)$ being concave, monotone, and increasing.
Then, the proof is complete by Definition~\ref{def:3}.
\end{proof}


The main competitive ratio result of GADGET is stated in the following theorem.
Due to space limitation, we provide a proof sketch in this paper.
\begin{thm}\label{thm:greedy}
Algorithm~\ref{alg:fractional_scheduling} produces a schedule that is $\frac{\alpha}{\alpha+1}$- competitive, where $\alpha \in (0,1]$ is the approximation ratio of solving Problem~(\ref{problem:pt}) in each time-slot.
%(see Appendix~\ref{appdx:prop_ratio}).
\end{thm}

\begin{proof}[Proof Sketch]
The main idea of our proof is to leverage the $p$-system result for greedy algorithms with approximation, where $p$ denotes the ratio between the maximum and minimum cardinalities of maximal independent sets in a family of independent sets.
It has been shown (e.g., \cite{Calinescu11:matroid}) that applying an online greedy algorithm with an approximation ratio of $\alpha \!\in\! (0,1]$ in each round for a $p$-system yields a competitive ratio of $\frac{\alpha}{\alpha+p}$.
Hence, the result in Theorem~\ref{thm:greedy} is proved once we show that Problem~DDLJS is a 1-system ($p\!=\!1$).

Toward this end, recall that the space of all possible schedules $\mathcal{V}=\{y_{is}[t], \forall i, s, t\}$ is partitioned into a collection of disjoint ``allocations'' $\{\mathcal{V}[t]\}$, $t\in\mathcal{T}$, where $\mathcal{V}[t]=\{y_{is}[t], \forall i, s\}$ and the independence family is $\mathcal{J} = \{ \mathcal{H} \in \mathcal{V}: |\mathcal{H} \!\cap\! \mathcal{V}[t]| \!\leq\! 1, \forall t\}$.
For any $Y \!=\! \{\mathcal{U}[t] \!\subseteq\! \mathcal{V}[t], \forall t \} \!\subseteq\! \mathcal{V}$, let $\mathcal{B}(Y)$ be the set of maximal independent sets of $\mathcal{V}$ included in $Y$,
%Without loss of generality, we let $Y=\{\mathcal{U}[t]\subseteq \mathcal{V}[t]\}$, $\forall t$, 
which implies that $|\mathcal{H}\cap\mathcal{U}[t]| \leq 1$.
Then, we can show that $\mathcal{B}(Y)=\{\{u_k[t]\in\mathcal{U}[t], \forall t\},\forall k\}$, where $k$ is the element (scheduling) index in the set $\mathcal{U}[t]$.
Thus for any $A\in\mathcal{B}(Y)$, the cardinality of $A$ is the same (i.e., $|A|=|Y|$), which immediately implies that $p=1$ and the proof is complete.
%Note that exactly one scheduling (can be infeasible) will be selected at each time slot, i.e., exactly one element from $\mathcal{U}[t]$ will be selected.
\end{proof}

 
\subsection{Solving the Per-Time-Slot Problem in (\ref{problem:pt})} \label{sec:VNE}

Under the temporally greedy approach in Algorithm~\ref{alg:fractional_scheduling}, it remains to solve an NP-Hard problem in (\ref{problem:pt}).
Due to the challenges in directly handling the ring topological constraint in \eqref{ctr:cycle} that is mixed-integer and highly unstructured,
we take an ``indirect'' approach by noting that Problem~\eqref{problem:pt} is a {\em generalized} virtual network embedding (VNE) problem (embedding a virtual computational graph onto a substrate physical graph while respecting all capacity constraints).
Notably, VNE with request graphs of cactus-type topologies has been solved in~\cite{Rost18:VNE}, which includes the ring topology as a special case.
The basic idea of the solution is based on randomized rounding the routing graphs over the underlying multi-commodity flow (MCF) problem (see, e.g., \cite{Rost18:VNE,Raghavan85:graphrandomizedrounding} for details).

However, our work differs from standard VNE~\cite{Rost18:VNE} in the following two key aspects: 
1) Unlike in standard VNE where the number of nodes in each request graph is given, the  number of nodes (i.e., workers) is part of the problem in \eqref{problem:pt}; 
2) Unlike standard VNE with a one-dimensional resource capacity constraint, Problem~\eqref{problem:pt} has  {\em multi-dimensional} resource capacity constraints.
Due to these differences, we refer to Problem~\eqref{problem:pt} in this paper as the {\em generalized} VNE (G-VNE).
%In contrast to the standard VNEP where the node number of each request graph is given, the best number of nodes (i.e., workers) should be determined before the VNEP solver can be leveraged in our case.

To address these challenges, we again take a {\em ``divide-and-conquer''} approach:
i) We observe that, although the number of workers is unknown, its upper bound $q_i[t]$ can be obtained efficiently by solving Problem~(\ref{problem:pt}) with continuous relaxations of Constraints (\ref{ctr:maxworker}), (\ref{ctr:cap}), and (\ref{ctr:iter_t});
ii) Once the upper bound of the number of workers is known, we can reformulate the G-VNE problem with a ``one-hot'' worker number constraint.

To reformulate the G-VNE problem, we let $\rho_i[t] \!\in\!\{0,1\}$ be the binary variable to indicate whether job $i$ is embedded in time slot $t$.
Let $\mathcal{Q}_i[t] \triangleq \{1, \ldots, \lceil q_i[t] \rceil \}$ be the set of all possible numbers of workers at time t for job $i$.
Let binary variable $\chi_{i,\kappa}[t] \in \{0,1\}$ denote whether a ring of size $\kappa \in\mathcal{Q}_i[t]$ is chosen at time $t$.
We use $V_i^\kappa$ and $E_i^\kappa$ to represent the sets of nodes and edges of the chosen $\kappa$-ring, respectively.
Let $\varrho^u_{i, \kappa,a}[t]$ and $\theta^{u,v}_{i,\kappa,a,b}[t]$ denote whether node $a\in V^\kappa_i$ and edge $(a,b)\!\in\!E^\kappa_i$ are mapped to a physical node $u\!\in\!V_s$ and a physical link $(u, v)\in E_s$ at time $t$, respectively.
%We also use  to denote whether an edge $(a,b)\in E^\kappa_i$ is mapped to a physical link $(u, v)\in E_s$ at time $t$.

Next, we use $d_{i,\kappa}^{a, r}$ and $d_{i,\kappa}^{a,b}$ to denote the type-$r$ resource demand for node $a\in V_i^{\kappa}$ and resource demand for edge $(a,b)\in E_i^{\kappa}$ in the chosen $\kappa$-ring of job $i$, respectively.
Let $g_s^{u,r}$ and $e_s^{u,v}$ be the type-$r$ resource capacities of node $u\in V_s$ and edge $(u,v)\in E_s$ in the substrate network, respectively.
%
Also, let $h_i^{u,r}[t]$ and $o_i^{u, v}[t]$ denote the cumulative type-$r$ resource allocation on node $u$ and the cumulative and aggregated resource allocation on edge $(u,v)$ of job $i$ in the substrate network at time $t$, respectively.
Let $\pi_{i,\kappa}[t]$ be the incremental utility with the $\kappa$-ring chosen at time $t$, i.e., $\pi_{i,\kappa}[t]=\mu_i(\zeta_iz_{i,t-1}+\zeta_i \sum_{\kappa \in \mathcal{Q}_i[t]} \kappa \chi_{i,\kappa}[t]  -\mu_i(\zeta_iz_{i,t-1})$.
% where $q_{i, \kappa}[t]$ is the number of workers of the chosen $\kappa$-ring at time $t$.
%Our objective is to maximize the overall utility for a set of active jobs $\mathcal{I}[t]$.
We let $\delta^+(u)$ and $\delta^-(u)$ denote the sets of outgoing and incoming edges of a node $u$, respectively.
Then, the G-VNE problem in time-slot $t$ can be reformulated as an integer linear program (ILP) (omitting time index ``$[t]$''  for notational simplicity): 
\begin{align}
&\label{problem:mcf}\text{Maximize }
     \sum_{i\in\mathcal{I}}\sum_{\kappa\in\mathcal{Q}_i}\pi_{i,\kappa}\chi_{i,\kappa}\\
%    \text{subject to } 
    &\label{lp:1}\sum_{\kappa\in\mathcal{Q}_i}\chi_{i,\kappa} = \rho_i,\quad\forall i\in\mathcal{I},\\
    &\label{lp:2}\sum_{u\in V_s}\varrho^u_{i,\kappa,a}= \chi_{i,\kappa}, \quad \forall i\in\mathcal{I}, \kappa\in\mathcal{Q}_i, a\in V_i^\kappa, \\
    &\nonumber\label{lp:3}\sum_{\substack{(u,v) \in\delta^+(u)}} \theta^{u,v}_{i,\kappa, a, b} - \sum_{\substack{(v,u) \in\delta^-(u)}}\theta^{v,u}_{i,\kappa,a,b}= \varrho^u_{i,\kappa, a} -\varrho^u_{i,\kappa, b}, \\
    &\hspace{1in}\forall i\in\mathcal{I}, \kappa\in\mathcal{Q}_i, (a,b)\in E_i^\kappa, u\in V_s,\\
   &\label{lp:4} \sum_{\kappa\in\mathcal{Q}_i}\sum_{a\in V^\kappa_i}d_{i,\kappa}^{a,r} \varrho^u_{i,\kappa,a} = h_i^{u,r}, \quad \forall i\in\mathcal{I}, u\in V_s, r\in\mathcal{R},\\  
    &\label{lp:5}\sum_{\kappa\in\mathcal{Q}_i}\sum_{(a,b)\in E^\kappa_i}d_{i,\kappa}^{a,b} \theta^{u,v}_{i,\kappa,a,b} = o_i^{u,v}, \forall i\in\mathcal{I}, (u,v)\in E_s,\\ 
    &\label{lp:6}\sum_{i\in\mathcal{I}}h_i^{u,r}\leq g_s^{u,r}, \quad\forall u \in V_s,\forall r\in\mathcal{R},\\
    &\label{lp:7}\sum_{i\in\mathcal{I}}o_i^{u,v}\leq e_s^{u,v}, \quad\forall (u,v) \in E_s.
%    &\nonumber y_{is}[t]\geq 0, x_{is}[t]\!\in\!\{0,1\},\forall i\!\in\!\mathcal{I}[t], s\in\mathcal{S}\nonumber.
\end{align}
%It is a mixed integer linear programming, which uses binary variables to compute a single valid mapping for each request.
Here, Constraint~(\ref{lp:1}) ensures that at most one of the $\kappa$-ring graphs ($\kappa=1,\ldots,\lceil q_i \rceil $) from $\mathcal{Q}_i$ can be selected.
Constraint~(\ref{lp:2}) ensures that if job $i$ is embedded ($\rho_i=1$) and if a $\kappa$-ring graph is selected ($\chi_{i,\kappa}=1$), then each node $a\in V_i^\kappa$ must be mapped to some physical node in $V_s$, i.e., there exists a node $u\in V_s$ such that $\varrho_{i,\kappa,a}^u = 1$.
Constraint~(\ref{lp:3}) induces a non-splittable unit flow for each edge $(a,b)\in E_i^\kappa$ from the physical location that $a$ is mapped to the physical location that $b$ is mapped.
Constraints~(\ref{lp:4})--(\ref{lp:5}) compute the cumulative resource on physical nodes and edges, respectively.
Constraints~(\ref{lp:6})--(\ref{lp:7}) ensure no violation of the physical nodes and edges resource capacities, respectively.
%
%It becomes linear program by relaxing the binary variables to [0,1].
%and Constraint~(\ref{lp:1}) is equivalent to $\sum_{\kappa\in\mathcal{Q}_i}\chi_{i,\kappa}\leq 1$.
Note that Constraints~(\ref{lp:1}), (\ref{lp:4}) and (\ref{lp:6}) are the {\em major differences} from the MCF formulation of the standard VNE problem (see, e.g., \cite{Rost18:VNE}), where each job has only one request graph (i.e., $|\mathcal{Q}_i|=1$) and each node has only one resource type.

Now, consider a linear program (LP)-based ring selection approach:
Let $\{\bar{\chi}_{i,\kappa}, \bar{\rho}_i\}$ be the LP-relaxation solution of Problem~(\ref{problem:mcf}) and $\bar{\pi}_{i,k}$ be the its utility value.
%To maximize the objective function in Eq.~(\ref{problem:mcf}), 
Select $\kappa_i = \max_{\kappa\in\mathcal{Q}_i : \bar{\chi}_{i,\kappa>0}}\{\bar{\pi}_{i,\kappa}\bar{\chi}_{i,\kappa}\}$ as the request ring-graph of job $i$ for $\bar{\rho}_i>0$.
That is, we set $\chi_{i,\kappa_i}\!=\!1$ and $\chi_{i,\kappa}\!=\!0$ if $\kappa\!\neq\!\kappa_i$, for each job with $\bar{\rho}_i>0$.
%We then normalize $\bar{\chi}_{i,\kappa}$ to $\tilde{\chi}_{i,\kappa}$, i.e., make $\sum_{\kappa\in\mathcal{Q}_i}\tilde{\chi}_{i,\kappa}$ to 1.
%Since $\sum_{\kappa\in\mathcal{Q}_i}\tilde{\chi}_{i,\kappa}=1$, we use $\tilde{\chi}_{i,\kappa}, \forall \kappa\in\mathcal{Q}_i$ as a probability distribution, and select one $\kappa_i\in\mathcal{Q}_i$ accordingly. We set $\chi_{i,\kappa_i}=1$ and $\chi_{i,\kappa}=0$ if $\kappa\neq\kappa_i$, for each job $i\in\mathcal{I}$.
%We next prove in Theorem~\ref{thm:randomized} that the approximation ratio of this scheme enjoys a ratio that not depends on the problem size.
Then, we can show that this LP-based ring selection scheme has the following approximation ratio:
%We next state the approximation ratio of this LP-based selection scheme in Lemma~\ref{lem:selection}.

\begin{lem}[LP-based Ring Selection]\label{lem:selection}
%Let $n_i=\min\{N_i, q_i\}$, then the selection scheme achieves at least  $\min_i1/n_i$ fraction of the utility obtained by some offline optimal approach.
Let $\Gamma\!\!=\!\!\max_i \lceil q_i\rceil$.
The LP-based ring selection scheme achieves at least  a $1/\Gamma$-fraction of the utility obtained by an offline optimal approach.
\end{lem}
\begin{proof}
Let $\chi^*_{i,\kappa^*}$, $\pi^*_{i,\kappa^*}$ be the optimal solution and objective value with $\kappa^*$ being the optimal ring size, respectively.
Let $\hat{\chi}_{i,\hat{\kappa}}$, $\hat{\pi}_{i,\hat{\kappa}}$ be the solution and objective value of our LP-based scheme, respectively, with $\hat{\kappa}$ being the ring size of the LP-based scheme.
Let $\Pi_i\triangleq\min\{N_i,\frac{C_s^r}{l_i^r},\frac{F_i^r}{l_i^r}, \forall r,s \}, \forall i$.
Then, 
\begin{align*}
&\frac{\sum_i\pi^*_{i,\kappa^*}\chi^*_{i,\kappa^*}}{\sum_i\hat{\pi}_{i,\hat{\kappa}}\hat{\chi}_{i,\hat{\kappa}}}\leq\frac{\sum_i\sum_\kappa\bar{\pi}_{i,\kappa}\bar{\chi}_{i,\kappa}}{\sum_i\hat{\pi}_{i,\hat{\kappa}}\hat{\chi}_{i,\hat{\kappa}}}\overset{(a)}{\leq}\max_i\frac{\sum_\kappa\bar{\pi}_{i,\kappa}\bar{\chi}_{i,\kappa}}{\hat{\pi}_{i,\hat{\kappa}}\hat{\chi}_{i,\hat{\kappa}}}\overset{(b)}{\leq}\Gamma.
\end{align*}
To see why $(a)$ holds, let $\bar{\iota}_i\triangleq\sum_\kappa\bar{\pi}_{i,\kappa}\bar{\chi}_{i,\kappa}$ and $\hat{\iota}_i\triangleq \hat{\pi}_{i,\hat{\kappa}}\hat{\chi}_{i,\hat{\kappa}}$.
Let $i^* = \arg\max_{i} \big\{ \frac{\sum_\kappa\bar{\pi}_{i,\kappa}\bar{\chi}_{i,\kappa}}{\hat{\pi}_{i,\hat{\kappa}}\hat{\chi}_{i,\hat{\kappa}}} \big\}$.
%That is $\frac{\bar{\iota}_{i^*}}{\hat{\iota}_{i^*}}\geq \frac{\bar{\iota}_i}{\hat{\iota}_i}, \forall i$.
Thus, we have
$\frac{\bar{\iota}_{i^*}}{\hat{\iota}_{i^*}} - \frac{\sum_i\bar{\iota}_i}{\sum_i\hat{\iota}_i}=\frac{\bar{\iota}_{i^*}\sum_i\hat{\iota}_i-\hat{\iota}_{i^*}\sum_i\bar{\iota}_i}{\hat{\iota}_{i^*}\sum_i\hat{\iota}_i} \!=\! \frac{\sum_i(\bar{\iota}_{i^*}\hat{\iota}_i-\bar{\iota}_i\hat{\iota}_{i^*})}{\hat{\iota}_{i^*}\sum_i\hat{\iota}_i} \!\geq\! 0$. 
Also, $(b)$ follows from i) the LP relaxation: $\frac{\bar{\pi}_{i,\kappa}\bar{\chi}_{i,\kappa}}{\hat{\pi}_{i,\hat{\kappa}}\hat{\chi}_{i,\hat{\kappa}}} \!\leq\! 1, \forall i, \forall \kappa \!\in\! \mathcal{Q}_i$); and ii) $|\mathcal{Q}_i| \!=\! \lceil q_i\rceil \!\leq\! \Pi_i$.
This completes the proof.
\end{proof}


Next, upon determining the ring size $\kappa$, we perform virtual network embedding with multi-dimensional resource constraints.
%Firstly, the LP solution with $\kappa=\hat{\kappa}$ is decomposed into a convex combinations of mappings, and each mapping is picked probabilistically with their weights (Algorithm~1 in~\cite{Rost18:VNE}).
% which includes following three steps: i) Solving original problem with integer relaxation; ii) Decomposing the solution into a convex combinations of mappings; and iii) Probabilistically picking the mapping with their weights.
First, similar to \cite[Formulation~2]{Rost18:VNE}, we resolve the uncertainty that may occur in embedding cyclic graphs by creating an augmented LP \cite{Rost18:VNE} that binds multiple copies of a ``reduced version'' of Problem~(\ref{problem:mcf}), where the set of $\hat{\kappa}$-rings has been chosen following the LP-based ring selection.
Then, we solve the augmented LP to obtain a relaxation solution, which can be used to recover a set of mapping-selection tuples $\mathcal{M}_i=\{(\varphi_i^k, \omega_i^k), k=1,\ldots,|\mathcal{M}_i| : \varphi_i^k>0, \sum_{k} \varphi_i^k \leq1 \}$ for each job $i$, where the mapping $\omega_i^k$ (a candidate of embedding) is chosen with probability $\varphi_i^k$, and rejected with probability $1-\sum_k\varphi_i^k$.
Note that to address the {\em multi-dimensional resource} challenge in computing $\mathcal{M}_i$, our key idea is to conduct mapping search to determine $\omega_i^k(r)$ for each $r \in \mathcal{R}$ by leveraging techniques in \cite[Sec.~III-C]{Rost18:VNE}.
Then, we choose $\omega_{i}^{k}\!=\!\cap_{r\in\mathcal{R}}\omega_{i}^{k}(r)$.
%we determine $\omega_i^k$  by choosing the bottleneck resource.
After the set $\{ \mathcal{M}_i, \forall i \}$ is calculated, we perform randomized rounding with probabilities based on $\varphi_i^k$-values  to obtain the embedding.
Putting all these together, we summarize our LP-based ring-selection and multi-dimensional resource embedding (LP-RS-MDE) method in Algorithm~\ref{alg:round}.
\begin{algorithm}
\SetAlgoLined
% \KwResult{The $\epsilon$-approximation fractional solution for each job $i$. }
\label{line:intialization}\textbf{Initialization:} Choose $u_b$ as the maximum number of roundings, and set $iter\leftarrow 1$\;
%
Set the values of constants $\alpha$, $\beta^r$, $\gamma$  (see Theorem~\ref{thm:ratio})\;
%\For{$i\in\mathcal{I}[t]$}{\label{line:lp_start}
%	Solve Problem~(\ref{problem:lp2}) with the goal to maximize $x'_i$\;
%	Remove job $i$ from set $\mathcal{I}[t]$ if $x'_i<1$\;
%}
%Solve Problem~(\ref{problem:lp2}) for the updated $\mathcal{I}[t]$\label{line:lp_end}\;
Solve the LP relaxation of Problem~(\ref{problem:mcf}) and set ring sizes $\kappa_i = \max_{\kappa\in\mathcal{Q}_i : \bar{\chi}_{i,\kappa>0}}\{\bar{\pi}_{i,\kappa}\bar{\chi}_{i,\kappa}\}$ for all job $i$\label{line:LP1}\;
Solve an augmented LP  with ring sizes fixed in Step~\ref{line:LP1}\label{line:LP2}\;
\For{$i\in\mathcal{I}[t]$}{\label{line:dmp_start}
	Compute $\mathcal{M}_i\!\!=\!\!\{(\varphi_i^k,\omega_i^k)\}$ based on the solution of the augmented LP, where $\varphi_i^k, \omega_i^k$ are determined by \cite[Sec.~III-C]{Rost18:VNE} and the bottleneck resource\label{line:dmp_end}\;
}
\While{solution is not $(\alpha, \beta^r, \gamma)$-approx. \& $iter\!<\!u_b$}{\label{line:round_start}
	{\bf foreach} $i\in\mathcal{I}[t]$ choose $\omega_i^k$ with probability $\varphi_i^k$\;
	$iter\leftarrow iter + 1$\label{line:round_end}\;
	
}
 \caption{LP-based Ring-Selection and Multi-Dimensional Resource Embedding (LP-RS-MDE).}
 \label{alg:round}
\end{algorithm}


%Toward this end, %we let $\epsilon\in(0,1]$.
To analyze LP-RS-MDE's performance, we let $d^r_{max}(i, u)$ and $d_{max}(i, u, v)$ denote the maximal type-$r$ resource demands that job $i$ imposes on node $u$ and edge $(u,v)$ in the substrate network, respectively.
Let $C^r_{max}(i, u)$ and $C_{max}(i, u, v)$ denote the maximal type-$r$ resource allocation that a valid mapping of job $i$ may impose on the substrate network's nodes and edges, respectively.
We define two constants as follows:
\begin{align*}
&\Delta^r(V_s) \triangleq \max_{u}\sum_{i\in\mathcal{I}[t]:d^r_{max(i,u)>0}}\!\!\!\!(C^r_{max}(i,u)/d^r_{max}(i,u))^2, \forall r,\\
&\Delta(E_s) \triangleq \max_{(u,v)}\sum_{i\in\mathcal{I}[t]:d_{max(i,u,v)>0}}\!\!\!\!\!\!(C_{max}(i,u,v)/d_{max}(i,u,v))^2.
\end{align*}

Also, we let $A^{u,r}[t]$ and $A^{u,v}[t]$ represent the overall type-$r$ resource allocation on node $u\in V_s$ and on edge $(u,v)\in E_s$ after randomized rounding at time $t$, respectively.
Then we have following analytical results:
\begin{thm}[Performance of LP-RS-MDE]
\label{thm:ratio} Assume that the substrate network has at least three servers ($|V_s|\geq 3$).
%, and the given request graph is cyclic.
%Let $\Omega$ be the overall utility obtained by our algorithm~\ref{alg:round}, and let $\Omega_{IP}$ be the optimal overall utility obtained by an optimal algorithm.
%Then, we have $\mathds{P}(\Omega<1/3\cdot\Omega_{IP})\leq \exp(-2/9)$.
Then, LP-RS-MDE achieves at least %a least 
$(1/3)$-fraction of the optimal value of Problem~\eqref{problem:mcf}, with probabilities of resource constraint violations satisfying $\mathbb{P}\{A^{u,r}[t] \geq \beta^rg_s^{u,r}\} \leq |V_s|^{-4}, \forall r, u, t$, and $\mathbb{P}\{A^{u,v}[t]\geq \gamma e_s^{u,v}\}\leq |E_s|^{-4}, \forall (u,v), t$, where $\beta^r =1+\epsilon\sqrt {2\Delta^r(V_s)\log(|V_s|)}$, $\forall r$, and $\gamma = 1 + \epsilon\sqrt{2\Delta(E_s)\log(|E_s|)}$.
\end{thm}

To prove Theorem~\ref{thm:ratio}, note that unlike the single-dimensional resource capacity in standard VNE~\cite{Rost18:VNE}, the analysis of Algorithm~\ref{alg:round} needs to consider multi-dimensional resource capacity violation (see Eqs.~(\ref{lp:4}) and (\ref{lp:6})).
Toward this end, we observe that the mapping computation in Step~\ref{line:dmp_end} of Algorithm~\ref{alg:round} implies that a similar approach as in \cite{Rost18:VNE} can be used to analyze the final mapping for each type-$r$ resource in each job, which in turn leads to the results stated in Theorem~\ref{thm:ratio}.
We omit the proof details here due to space limitation.
Next, we analyze the running time complexity of LP-RS-MDE.

\begin{thm}[Time Complexity of LP-RS-MDE]\label{thm:time}
LP-RS-MDE has polynomial time complexity $O((|\mathcal{I}[t]|\cdot|G_s|)^3 + u_b\cdot\mathcal{I}[t])$.
%{\color{red}where $u_b$ is the maximal rounding numbers.}
\end{thm}

\begin{proof}
The main components of the running time include solving the LP relaxations to obtain fractional solutions (Lines~\ref{line:LP1}-\ref{line:LP2} in Algorithm~\ref{alg:round}), computing valid mappings using decomposition approach (Lines~\ref{line:dmp_start}-\ref{line:dmp_end} in Algorithm~\ref{alg:round}), and then performing randomized rounding on these computed mappings (Lines~\ref{line:round_start}-\ref{line:round_end} in Algorithm~\ref{alg:round}). %\kliu{on what?}.
The time complexity of solving the LP relaxations is $O((|\mathcal{I}[t]| \cdot |G_s|)^3)$~\cite{VaidyaLP:90}.
The mapping search step terminates when $\varrho_i \leq 0$, and in each termination, at least one variable becomes $0$.
The number of variables for each job $i$ is bound by $O(|G_i| \cdot |G_s|)$ for each copy of Problem~(\ref{problem:mcf}).
Specifically, the mapping search visits all nodes and edges in the request graph.
Also, in each visit, in order to find the set of mapping-selection tuples $\{ \mathcal{M}_i$, $\forall i\}$, the substrate network will be traversed.
% using BFS. %according to Lemma~\ref{lem:connectivity}
Thus, the total number of variables is upper bounded by $O(|G_i| \cdot |G_s|)$.
Further, there are at most $O(|V_s|)$ copies of Problem~\eqref{problem:mcf}, which implies $O(|G_i|\cdot|G_s|\cdot |V_s|\cdot|\mathcal{I}[t]|)$ complexity.
%
Finally, the rounding time of each job $i$ is bounded by $u_b$, and thus the running time is bounded by $O(u_b\cdot\mathcal{I}[t])$. %\kliu{Can't find the definition of $u_b$.}
Hence, the overall time complexity of the LP-RS-MDE method is $O((|\mathcal{I}[t]|\cdot|G_s|)^3\!+\!u_b\cdot\mathcal{I}[t])$, and the proof is complete.
\end{proof}

%\section{Performance Analysis}
By combining results in Theorems~\ref{thm:greedy} and \ref{thm:ratio}, we have: 

\begin{thm}[Competitive Ratio of GADGET]\label{thm:overallratio}
Algorithm~\ref{alg:fractional_scheduling} produces a schedule that yields a utility value at least  $(\frac{1}{3\Gamma+1})$-fraction of the maximum utility value of Problem~DDLJS, with probabilities of resource violations satisfying $\mathbb{P}\{A^{u, r} [t] \geq \beta^r g_s^{u,r}, \exists t \in \mathcal{T} \} \leq 1-(1-|V_s|^{-4})^T, \forall u, r$, and $\mathbb{P}\{A^{u, v} [t] \geq \gamma e_s^{u,v}, \exists t \in \mathcal{T} \} \leq 1-(1-|E_s|^{-4})^T, \forall (u,v)$, where $\Gamma$ and $\beta^r$, $\gamma$ are as defined in Lemma~\ref{lem:selection} and Theorem~\ref{thm:ratio}.
%And $\Gamma$ is defined as in Lemma~\ref{lem:selection}.
\end{thm}


















==> AllReduce_Scheduling_INFOCOM'21/Sec6-Numerical/Sec6-Numerical.tex <==
% !TEX root = ../AllReduce-Scheduling-INFOCOM'21.tex

\begin{figure*}[t!]
 \begin{minipage}[t]{0.24\linewidth}
%        \centering
        \includegraphics[width=1.1\textwidth]{Figures/jobvaried-eps-converted-to.pdf}
        \caption{Total utility comparisons.} \label{fig:utility}
    \end{minipage}%
    \hspace{0.005\linewidth}
    \begin{minipage}[t]{0.24\linewidth}
        \centering
        \includegraphics[width=.96\textwidth]{Figures/NRF-eps-converted-to.pdf}
        \caption{Embedded ratio overview w.r.t node resource.} \label{fig:NRF}
    \end{minipage}%
    \hspace{0.005\textwidth}
    \begin{minipage}[t]{0.24\linewidth}
%        \centering
        \includegraphics[width=1.1\textwidth]{Figures/ERF-eps-converted-to.pdf}
        \caption{Embedded ratio overview w.r.t edge resource.}\label{fig:ERF}
    \end{minipage}%
    \hspace{0.005\linewidth} 
    \begin{minipage}[t]{0.24\linewidth}
%        \centering
        \includegraphics[width=1.1\textwidth]{Figures/ratio-eps-converted-to.pdf}
        \caption{%Embedding 
		Approximation ratio.}\label{fig:ratio}
    \end{minipage}%
\vspace{-.2in}
\end{figure*}



\section{Empirical Studies}%Numerical Results
\label{sec:numerical}


In this section, we conduct simulations to evaluate our GADGET algorithm.
We use ``excessive training avoidance'' as an application example (cf. Section~\ref{sec:general_framework}, Page~5), which aims to maximize the overall utility in a GPU computing cluster.
%\footnote{We do not consider overall resource constraint in the cluster, as a cloud typically provides sufficient resources for serving a large number of customers.} 
%under the setting that the resource is not reserved for each job, i.e., $l_i^r$ is not given by the user and the system will dynamically allocate resources to jobs to maximize the overall utility.
Here, Eq.~(\ref{ctr:iter}) is specialized to $\sum_{t}\sum_{s}y_{is}[t]\leq F_i,\forall i$, where $F_i$ is the maximum number of iterations specified by users upon their job submissions.
Eq.~(\ref{ctr:cap}) is specialized to $\sum_i y_{is}[t] \!\leq\! C_s, \forall s, t$, where $C_s$ is the GPU capacity of server $s$.

\smallskip
{\bf 1) Experiment Settings:} We use a ``fat-tree'' GPU computing cluster running for $T\!=\!200$, with $S\!=\!50$ servers.
% $T = 200$ time slots, with $S=50$ servers to host workers.
The servers are randomly divided into ``racks'' and the number of racks is randomly chosen between $[2, 5]$.
Following similar settings as in~\cite{Mahajan20:Themis}, we configure each server with the number of GPUs randomly chosen from the discrete set $\{1, 2, 4, 8\}$.
We adopt the job arrival pattern from the Google Cluster data~\cite{Reiss12:googlecluster}.
%but with normalized job arrival rates in alternating time-slots as follows: the arrival rates are $1/3$ and $2/3$ in odd and even time-slots, respectively.
The job parameters are integers generated uniformly at random from the following intervals: $N_i\!\!\in\!\![1, 5]$, $F_i\!\in\![1000,6000]$, $\zeta_i\!\in\![50,500]$, and $b_i\in[100 \text{ Mbps}, 5 \text{ Gbps}]$.
The bandwidths between racks and servers are chosen from $[200 \text{ Gbps}, 3200 \text{ Gbps}]$~\cite{Scott:bandwidth} and $[10 \text{ Gbps}, 100 \text{ Gbps}]$ uniformly at random, respectively.
We adopt the Sigmoid utility function~\cite{Huang15:CORA}: $\mu_i(y_{is}[t]) = \frac{\lambda_{i,1}}{1+e^{-\lambda_{i,2}(\zeta_i\sum_{s\in\mathcal{S}}y_{is}[t]+\zeta_iz_{i,t-1}-\lambda_{i,3})}}$, where $\lambda_{i,1}\in[1,100]$ represents the priority of job $i$, $\lambda_{i,2} \!\in\!(0,1)$ is to represent the sensitivity of the job to the number of iterations, and $\lambda_{i,3}\in[300, 3000]$ represents the expected number of iterations that should be trained.

\smallskip
{\bf 2) Baselines:} We compare GADGET with the following representative job scheduling policies for computing clusters:

\begin{list}{\labelitemi}{\leftmargin=1em \itemindent=-0.09em \itemsep=.2em}

\item {\em FIFO in Hadoop and Spark~\cite{Zaharia10:Spark}:} Jobs are scheduled in the order of their arrivals with a fixed number of workers. 

\item {\em Dominant Resource Fairness Scheduling (DRF) in Yarn~\cite{Vavilapalli13:Yarn} and Mesos~\cite{Hindman11:Mesos}:} Jobs are scheduled based on their dominant resource share.
%  to achieve the max-min fairness. 

\item {\em Least Attained Service (LAS) in Tiresias~\cite{Gu19:Tiresias}:} Resource scheduling among active users in the cluster is conducted in a round-robin fashion across jobs, according to the total number of accelerator hours consumed by each job.
\end{list}
Since the above scheduling policies do not consider the underlying topology constraints, we place workers based on the simple heuristic that greedily allocates workers to servers. %servers to workers 
where a cycle can be attained.
%We employ a round-robin approach to place workers on available machines in Baselines (1) and (2).
For FIFO and Tiresias, the number of workers is fixed to a number within $[1,10]$.

\smallskip
{\bf 3) Experiment Results:}
Fig.~\ref{fig:utility} illustrates the comparisons of our GADGET algorithm to the above baselines.
We can see that GADGET algorithm significantly outperforms the baseline algorithms, and the gains in total utility value over the baselines become more pronounced as the number of jobs increases.
%Also, DRF has better performance compared to FIFO and Tiresias since it can dynamically adjust the number of workers based on job's resource occupation.
This shows that the dynamic resource allocation in GADGET achieves higher resource utilization than those of the static resource allocations (i.e., the number of workers remains fixed throughout the training process) in the baselines.
%Note that higher workload jobs arrive earlier can introduce delay to later-joining smaller size jobs, which becomes worse if the scheduling time slot is chosen relatively large.
%We observe that the heuristic placement of workers to form a cycle can have a huge impact on the final obtained utility.

Next, we examine the impacts of node GPU and edge bandwidth resource capacities in the substrate network on the performance of GADGET.
The results are shown in Figs.~\ref{fig:NRF} and \ref{fig:ERF}, where one unit of node and edge resource in the y-axes represents (GPU=100, bandwidth=200Gbps).
% \textcolor{purple}{Wu: clarify what the y labels `Factor of units node resource' and `Factor of units edge resource' mean}
We evaluate the ratio between the numbers of embedded jobs and active jobs in each time slot, and the results in Figs.~\ref{fig:NRF} and \ref{fig:ERF} are the average ratio over three trials. %\kliu{how many trials?}. %all per-slot values.
We can see that increasing the node and edge capacities in the cluster has a positive impact, which allows more jobs to be embedded in each time slot.
Intuitively, as the GPU capacity of each node increases, jobs with high bandwidth demands have a higher probability to be allocated using intra-server communication, which typically has a much larger bandwidth capacity than that of inter-server communication.
Also, the larger the GPUs number, the more jobs can be trained simultaneously.
Similarly, the larger the edge capacity, the more jobs with inter-server communications can be scheduled.

%more changes \kliu{What do you mean ``changes'?'} for jobs to take advantage of inter-server communications, especially jobs with large bandwidth demands.
%Otherwise, these jobs can not be run in the absence of intra-sever communication support.

 
 
Lastly, we investigate the performance of our proposed G-VNE technique, which is a major component of our GADGET algorithm.
We evaluate the embedding performance in terms of the ratio between the total utility obtained by our algorithm and the optimal total utility.
The optimal utility of Problem~(\ref{problem:mcf}) at each time slot is computed using the global optimization solver Gurobi based on the branch-and-bound approach (of exponential complexity) \cite{Kobayashi20:branch_and_bound}.
%We vary the number of jobs from 10 to 50.
The results are shown in Fig.~\ref{fig:ratio}.
We can see that the actual performance ratio is better than our theoretical bound in Theorem~\ref{thm:ratio}, which achieves 60\%--80\% of the optimal utility obtained by the global optimization solver.



==> AllReduce_Scheduling_INFOCOM'21/Sec7-Conclusion/Sec7-Conclusion.tex <==
% !TEX root = ../AllReduce-Scheduling-INFOCOM'21.tex


\section{Conclusion}
\label{sec:conclusion}
In this paper, we studied online resource scheduling for the training of RAR-based DDL jobs in computing clusters.
We first developed an analytical optimization framework and then developed an online scheduling algorithm called GADGET
%, where we developed a performance provable greedy scheduling approach. 
In GADGET, by showing the temporal submodularity of the online scheduling problem, we developed a greedy scheduling approach with competitive ratio guarantee.
Then, for the NP-Hard subproblem in each time-slot, we proposed a generalized virtual network embedding technique with approximation ratio guarantee.
Trace-driven simulations confirmed the superior performance of GADGET over existing schemes.~\footnote{The authors have provided public access to their code or data at \url{https://zenodo.org/record/5847644#.YervbxNKhTZ}.}
%Collectively, our results serve as a fundamental building block toward scheduling optimization for RAR-based DDL jobs\footnote{The authors have provided public access to their code or data at https://zenodo.org/record/5847644\#.YeHePxNKhTY.}.
%All-reduce based DDL training scheduling remains an under-explored area.
%Future directions may include %, e.g., to 
%considering other all-reduced-based DDL scheduling beyond the ring topology.

==> AllReduce_Scheduling_INFOCOM'21/Supporting-Preambles/jackmac.tex <==
%>From snoeyink%cs.ubc.ca@cs.Technion.AC.IL Wed Nov  3 08:18:27 1993
%Received: from csmail.cs.technion.ac.il by math.tau.ac.il (5.67/math.tau-930921)
	%id AA17625; Wed, 3 Nov 93 08:18:23 +0200
%Received: from csc (csc.cs.technion.ac.il) by csmail.cs.Technion.AC.IL (4.1/3.14)
	%id AA14244; Wed, 3 Nov 93 01:19:10 IST
%Received: from csa by csc (4.1/3.14)
	%id AA24688; Wed, 3 Nov 93 01:19:48 IST
%Received: from grolsch.cs.ubc.ca by csa (4.1/3.14)
	%id AA20525; Wed, 3 Nov 93 01:11:28 IST
%Return-Path: <snoeyink@cs.ubc.ca>
%Received: from cascade.cs.ubc.ca by grolsch.cs.ubc.ca with SMTP id AA13516
  %(5.65c/IDA-1.3.5 for alon@cs.Technion.AC.IL); Tue, 2 Nov 1993 13:56:34 -0800
%Date: Tue, 2 Nov 1993 13:56:34 -0800
%From: Jack Snoeyink <snoeyink%cs.ubc.ca@cs.Technion.AC.IL>
%Message-Id: <199311022156.AA13516@grolsch.cs.ubc.ca>
%Received: by cascade.cs.ubc.ca (4.1/SMI-4.1)
	%id AA21873; Tue, 2 Nov 93 13:56:33 PST
%To: alon@cs.Technion.AC.IL
%In-Reply-To: Alon Efrat's message of Sun, 31 Oct 93 23:38:48 IST <9310312138.AA19880@csc>
%Subject: LaTex Macros
%Status: RO
%Content-Length: 19065
%X-Lines: 638
%
%
%I'm in oberwolfach w/ micha, so I';ll just send you this and answer
%your questions on it when I get back to vancouver next week...
%
    %o                                    Jack
  %_/\_.
%(')>-(`)                          snoeyink@cs.ubc.ca
%----figbox.tex----

% 12 Oct 90 LaTeX figure boxing macros  by Jack Snoeyink
%					w/ ideas from John Hershberger
%					and code from Tom Rokicki
%%%%%%%%%%%%%%%%%
% 
% This file contains two classes of macros for dealing with figures in
% Latex documents:  
%  \figbox (and its relatives) take a box containing a figure or table
%    or whatever, caption it, and either place it on the page and wrap the
%    text around it or let it float (as usual).
%  \boxeps and \boxps take encasulated or plain postscript from a file
%    and put it in a box for use by \figbox
%
%%%%%%%%%%%%%%%%
%
% The most important macro for dealing with boxes is:
%
% \figbox: caption a box as a figure or table and place it in the margin
% 	(a marginal box) or float it (a floating box).
% 	Wide marginal boxes are promoted to one column floats; wide one
% 	column floats are promoted to two column floats.
%
% Usage: \figbox [*htblr] {box} {style} {label} {caption}
%
% The optional argument default is [htb].  Other choices
%   * two column (must come first),
%   h here, t top, b bottom (as in latex),
%   l left, r right (marginal boxes that do not float)
%
% NB: Left and right marginal boxes will not overlap in height.
%
% Two column figures default to htb unless some other 
%   	options follow the *.
%   They can also be specified by style {figure*} or {table*}.
%
% box is a box containing a figure or table.
% style is the caption style {figure}, {figure*}, {table}, or {table*}.  
% label is the label assigned.
%	if empty, the figure will not be labeled.
% caption is of the form {}, {Caption} or {[short caption] Long caption},
%       where the short caption goes into the list of figures/tables.
%	if empty, the figure will not be captioned or labeled.
% 
% The lower level macro \captionbox, described much later, can be used
% to combine two or more captioned figures into a single marginal or
% floating box.
%
%%%%%%%%%%%%%%%%
%
% options defined by macros are: \captionstyle \boxcaptionstyle
% \maxfigfraction \figboxhang \figboxmargin 
%
% \captionstyle is executed for all floating box captions
% \boxcaptionstyle is executed for all marginal box captions.
%	Default \raggedright
% \maxfigfraction is the maximum fraction of a column that can be taken up
% 	by a marginal box before it gets converted to a float.
% 	Default .6
% dimen \figboxhang is the distance a marginal box hangs into the margin.
%	Default 0pt
% dimen \figboxmargin is the width of space between the text and a
% 	marginal box. 
%	Default .15in
%
%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%
%
% The most important macros for turning postscript into boxes are:
% 
% \boxeps: Form a box containing encapsulated postscript from a file at a
%	given scale.
% \boxps: Form a box containing postscript from a file at a given scale, 
% 	width, and height.
% 
%
% Usage: \boxeps[local commands] {file} {scale}
%	 \boxps[local commands] {file} {scale} {width} {height}
%
% The optional local commands are executed after scaling. As described
% 	below, they are useful for setting origins, non-uniform scaling, etc?
% file is the filename in the \figuredirectory and without the .ps
% 	extension.
% scale is a real number: 1 to use the drawn size.  0.9 to use 90% of
% 	drawn size.  Can be changed by local commands. (see below)
% width and height are dimensions of the box produced by \boxps.
%
%%%%%%%%%%%%%%%%
%
% options: \DVIscaling \figuredirectory \missingfigure \boxer
% local commands: \horizscale \vertscale
%
% \DVIscaling is the number the dvi to ps converter considers a unit
% 	scaling transformation.  Default: 1 for dvi2ps  --- 100 for
% 	some of Rokicki's versions of dvips.
%
% \globalscaling is the scaling applied to every picture --- useful
% 	for making double size figures for journals.  Default: 1
%
% \figuredirectory is the pathname where figure postscript files are kept.
%	Default: ./figure
%
% \missingfigure{file} is executed when the file is not found.
%	Default: \def\missingfigure#1{\hbox{Missing figure #1.ps}}
%
% \boxer is the command used by \boxps to make a box of the desired size
% 	containing the figure.  Possible commands depend on the origin of
% 	the figure, and include \llboxer \lcboxer \ulboxer and \ccboxer.
% 	(ll = lower left, ul = upper left, cc = dead center, etc.)
%	\boxer can be defined in the local commands or globally.
%
% Local commands \horizscale, and \vertscale can scale the picture
% 	horizontally and vertically by different factors.  \scale
% 	scales the picture uniformly.  Scales accumulate.
%
%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%
%
% Default options
%

\def\captionstyle{}
\def\boxcaptionstyle{\raggedright}

\def\maxfigfraction{.6}% 	--- max frac of column for marg figure

\newdimen\figboxmargin%		--- margin between text and picture
\figboxmargin = .15in

\newdimen\figboxhang%		--- amount to hang picture into margin
\figboxhang = 0pt

\def\DVIscaling{1}%		--- for dvi2ps
\def\globalscaling{1}%		--- for scaling everything
\def\figuredirectory{./figures}%--- where to find the .ps files 
\let\boxer=\llboxer%		--- default origin in lower left for non-
%				      encapsulated postscript figures

\def\missingfigure#1{\hbox{Missing figure #1.ps}}


%%%%%%%%%%%%%%%%
%
% Use latex internals
%
\catcode `\@=11
\special{! /@scaleunit 1 def }

\newbox\figurebox

\def\figbox{%	[place] box style label caption
\@ifnextchar[{\figboxaux}{\figboxaux[htb]}}

%
% Parse position parameters and try appropriate placement
%
\long\def\figboxaux[#1#2]#3#4#5#6{%	--- want left margin figure?
\writepict{{#3}{#4}{#5}{#6}}%		--- save figure if journalpicts
\setbox\figurebox\hbox{#3}%
\if l#1\tryleftbox{#4}{#5}{#6}%
\else%					--- want right margin figure?
\if r#1\tryrightbox{#4}{#5}{#6}%
\else%					--- want one or two column figure?
\if *#1\checktwocoloptions#2]{\box\figurebox}{#4*}{#5}{#6}%
\else\tryonecol[#1#2]{#4}{#5}{#6}%
\fi
\fi
\fi\ignorespaces}

%
% Try a placement; promote if too wide
%

\long\def\tryleftbox#1#2#3{%		--- does left margin figure fit?
\ifdim\wd\figurebox>\maxfigfraction\columnwidth \tryonecol[htb]{#1}{#2}{#3}%
\else\leftbox{\captionbox{\box\figurebox}{#1}{#2}{#3}}\fi}

\long\def\tryrightbox#1#2#3{%	--- does right margin figure fit?
\ifdim\wd\figurebox>\maxfigfraction\columnwidth \tryonecol[htb]{#1}{#2}{#3}%
\else\rightbox{\captionbox{\box\figurebox}{#1}{#2}{#3}}\fi}

\def\checktwocoloptions{%	--- make sure twocol has htb or p
\@ifnextchar]{\floatbox[htb}{\floatbox[}}

\long\def\tryonecol[#1]#2#3#4{%	--- does one column figure fit?
\ifdim\wd\figurebox>\columnwidth \floatbox[#1]{\box\figurebox}{#2*}{#3}{#4}%
\else\floatbox[#1]{\box\figurebox}{#2}{#3}{#4}\fi}

%
% Do the work for a floating box.
%
% \floatbox[place]{box} {style} {label} {caption}
%

\long\def\floatbox[#1]#2#3#4#5{%
\begin{#3}[#1]
\hbox to \hsize{\hfil#2\hfil}
\captionandlabel{#3}{#4}{#5}
\end{#3}
}


%
% Make a caption the width of the box with given style. 
%
%\captionbox {box} {style} {label} {[optshortcap] caption}
%
% options: \boxcaptionstyle 
%
%%%%%%%%%%%%%%%%
%
% This can be used with box commands (\hbox, \vbox, \mbox, and the like),
% along with \figbox with an empty caption, to place two or more captioned
% boxes in a single marginal or floating box.   
%
% e.g. \figbox{\hbox{
%		     \captionbox{ \boxeps{fig1}1} {figure} {f1} {a figure}
%		     \hskip 1in
%		     \captionbox{ \boxeps{tab1}1} {table} {t1} {a table}
%		    }} {figure} {ignored-label} {}
%

\long\def\captionbox#1#2#3#4{% box style label {[optshortcap] caption}
\setbox\figurebox\hbox{#1}%
\parbox[t]{\wd\figurebox}{%
\bigskip\box\figurebox
\let\captionstyle=\boxcaptionstyle
\captionandlabel{#2}{#3}{#4}
\bigskip
}}

%				--- caption and label if label is nonempty
\def\captionandlabel#1#2#3{% 	--- {style} {label} {caption}
\def\testit{#3}%
\ifx\testit\empty\else%		--- if non empty caption
\writecapt{{#1}{#2}{#3}}%	--- save for journal figs
\captypeunstarred#1*.%		--- remove optional stars
\getcaption#3\endc@ption%       --- parse the caption
\def\testit{#2}%		--- check for empty label
\ifx\testit\empty\else\label{#2}\fi
\fi}

\def\captypeunstarred#1*#2.{%	--- remove two-column star from style
\def\@captype{#1}}

%
% Parse the caption of the form {caption} or {[short] long caption} 
%

\def\getcaption{\@ifnextchar[{\getcaptwo}{\getcapone}}
\long\def\getcapone#1\endc@ption{\caption[#1]%
{\def\baselinestretch{1}\Large\normalsize\captionstyle\ignorespaces #1}}
\long\def\getcaptwo[#1]#2\endc@ption{\caption[#1]%
{\def\baselinestretch{1}\Large\normalsize\captionstyle\ignorespaces #2}}

%
% Do the right thing with an already captioned marginal box
%
% \leftbox{box}
% \rightbox{box}
%
% options: \figboxmargin \figboxhang \figuredirectory

\newdimen\figboxht
\newcount\figboxn


\newcount\figboxlines%		--- picture height in number of lines
\newdimen\figboxwid%		--- picture width

\newif\ifisleftbox

\long\def\leftbox#1{%
\setbox\figurebox\hbox{#1}\global\isleftboxtrue
\startmarginbox
\vadjust{\smash{\rlap{\hskip\hsize\hskip\figboxhang
\llap{\raise.7\baselineskip\box\figurebox\hskip\rightskip}}}}%
\endmarginbox%
}

\long\def\rightbox#1{%
\setbox\figurebox\hbox{#1}\global\isleftboxfalse
\startmarginbox
\smash{\llap{\raise.7\baselineskip\box\figurebox\hskip\figboxmargin}}%
\endmarginbox%
}

\def\startmarginbox{%
\ifvmode\passpict\let\endmarginbox=\indent
\else\message{WARNING: marginbox in not in vmode}\hfilneg\ \passpict
\let\endmarginbox=\relax\fi
%
\figboxht=\dp\figurebox%	 actual height
\advance\figboxht by 1.3\baselineskip% round up
\vskip\figboxht\penalty-300\vskip-\figboxht% filbreak trick
\divide\figboxht by\baselineskip%      how many lines?
\global\figboxlines=\figboxht
%
\global\figboxwid=\wd\figurebox
\global\advance\figboxwid by \figboxmargin
\global\advance\figboxwid by -\figboxhang
\setmypar\noindent}
%

%
% Useful macros
%
% for lengthening (and shortening) picture space
%
\def\addlines#1{\global\advance\figboxlines by #1\myparshape}
\def\zerolines{\origpar\global\figboxlines=0\myparshape}

%
% for passing any marginal figures
%
\def\passpict{\par\ifnum\figboxlines>1\vskip\figboxlines\baselineskip
\zerolines\fi}

\def\emptybox#1#2{\hbox to #1{\vbox to #2{\vss}\hss}}

%%%%%%%%%%%%%%%%%%%%%
%\par hacking  
% We define our own version of Tex's \par and tell Latex it is the original

\global\let\origpar=\@@par%	--- Latex's saved version of Tex's \par
\global\let\dopar=\origpar
\global\def\@@par{\dopar}
\@setpar{\dopar}

\def\setmypar{\global\let\dopar=\mypar
\global\prevgraf=0\myparshape}

\def\mypar{\origpar\global\advance\figboxlines by -\prevgraf%
\global\prevgraf=0\myparshape}

\def\myparshape{\relax%
\ifnum\figboxlines>1\theparshape \else
\global\hangindent=0pt\global\hangafter=1%  these sometimes get restored...
\global\let\dopar=\origpar\fi}

\def\theparshape{%
\ifisleftbox\global\hangindent=-\figboxwid 
\else\global\hangindent=\figboxwid \fi
\global\hangafter=-\figboxlines \global\advance\hangafter by 1%
}


%%%%%%%%%%%%%%%%
%
%  Macros to make the list of figures and captions used by journals
%
%  To use, execute \journalpicts{scalefactor} at the beginning of the
%  file.  All figbox figures and tables will be written to a .pic file
%  and all captions to a .cap file.  On \enddocument, these files are
%  read in and the lists of figures and captions are produced.
%  
%  For non-english versions, or to add other types of floats, the
%  macro \definefnum should be changed.
%

\def\definefnum#1{%		--- ugly latex hacking to get the
%		 			right figure/table name 
\def\fnum@figure{Figure \ref{#1}}%
\def\fnum@table{Table \ref{#1}}%
\def\fnum@code{Algorithm \ref{#1}}%
}

\def\writepict#1{}
\def\writecapt#1{}

%%%%%%%%%%%%%%%%
% \journalpicts{globalscalefactor} writes all pictures and captions to
% 	files and modifies \enddocument to read these files and
% 	produce lists of enlarged figures and of captions
% 

\def\journalpicts#1{% 		global scale factor
\newwrite\pictfile
\newwrite\captfile
%
\openout\pictfile\jobname.pic
\openout\captfile\jobname.cap
%
\gdef\writepict##1{\unexpandedwrite\pictfile{\doit##1}}%
\gdef\writecapt##1{\unexpandedwrite\captfile{\doit##1}}%
%
\global\let\ENDdocument=\enddocument
\gdef\enddocument{\DOjournalpicts{#1}\ENDdocument}
}

%
%	generate enlarged figures 1 per page and list captions
%
\def\DOjournalpicts#1{{%
\def\writepict##1{}\closeout\pictfile
\def\writecapt##1{}\closeout\captfile
\@fileswfalse%			--- turn off toc, lof, and so on.
%
\onecolumn
\def\globalscaling{#1}
\def\doit##1##2##3##4{%		--- print a picture on blank page
%					{box}{style}{label}{caption}
\figboxaux[t]{\hss##1\hss}{##2}{}{}%
\vspace*{1in}
\definefnum{##3}%		--- use Figure \ref{label} or Table \ref{label}
\captionandlabel{##2}{}{##4}
\clearpage}%
%
\input\jobname.pic
%
\def\doit##1##2##3{%		--- print caption
%					{style}{label}{caption}
\definefnum{##2}%		--- use Figure \ref{label} or Table \ref{label}
\captionandlabel{##1}{}{##3}}%
%
\raggedright\let\captionstyle=\raggedright
\def\@makecaption##1##2{##1: ##2\par}%  --- Be sure captions aren't centered
%
\input\jobname.cap
}}%				--- to be followed by \enddocument



%%%%%%%%%%%%%%%%
%
%  Box macros
%
%%%%%%%%%%%%%%%%
%
% \boxeps[local commands] {file} {scale}
%
% options \DVIscaling \figuredirectory \scale \horizscale \vertscale
% \missingfigure \globalscaling
%
% \boxps[local commands] {file} {scale} {width} {height}
%
% \scale \horizscale \vertscale 

%
%  Various `boxers' --- which one is used depends on where the origin
%  of the picture is.  If you are using the bounding boxes of
%  encapsulated postscript, just use the default \llboxer.  Otherwise,
%  you have to figure out where the origin is and set \boxer appropriately.
%

\def\llboxer#1{\vbox to \figboxht{\vfil\hbox to \figboxwid{#1\hfill}}}
\def\lcboxer#1{\vbox to \figboxht{\vfil\hbox to \figboxwid{\hfill#1\hfill}}}
\def\oldboxer#1{\vbox to \figboxht{\vfil
		      \hbox to \figboxwid{\hfill\llap{#1\hskip4.25in}\hfill}}}
\def\ulboxer#1{\vbox to \figboxht{\hbox to \figboxwid{#1\hfill}\vfil}}
\def\ccboxer#1{\vbox to \figboxht{\vfil
			\hbox to \figboxwid{\hfill#1\hfill}\vfil}}

% a macro to strip the pt off a dimension
%
{\catcode`\p=12\catcode`\t=12
\gdef\removedimen#1pt{#1}}

\def\defscaled#1#2{#2=\DVIscaling#2%
\xdef#1{\expandafter\removedimen\the#2}}

\def\DVIspace{ }
\newdimen\hscalefactor
\newdimen\vscalefactor

\def\scale#1{\horizscale{#1}\vertscale{#1}}
\def\horizscale#1{\hscalefactor=#1\hscalefactor\figboxht=#1\figboxht}
\def\vertscale#1{\vscalefactor=#1\vscalefactor\figboxwid=#1\figboxwid}

%%%%%%%%%%%%%%%%
%

\def\boxps{%
\@ifnextchar[{\boxpsaux}{\boxpsaux[\relax]}}

\def\boxpsaux[#1]#2#3#4#5{%
{\figboxwid#4\figboxht#5\hscalefactor=1pt\vscalefactor=1pt%
\scale{#3}%
\scale{\globalscaling}%
#1%
\defscaled\DVIhscale\hscalefactor
\defscaled\DVIvscale\vscalefactor
\boxer{\special{psfile=\figuredirectory/#2.ps \DVIspace
		hscale=\DVIhscale\DVIspace 
		vscale=\DVIvscale}}}%
}


%%%%%%%%%%%%%%%%
% The following is from tex/inputs/epsf.tex by Tom Rokicki
% with slight modifications by Jack Snoeyink.
%
%   Written by Tomas Rokicki of Radical Eye Software, 29 Mar 1989.
%
%   Include an ecapsulated postscript graphic.
%   Works by finding the bounding box comment.
%
\newread\Epsffilein
\newif\ifEpsffileok
\newif\ifEpsfbbfound

\newdimen\pspoints
\pspoints=1in
\divide\pspoints by 72


\def\boxeps{%
\@ifnextchar[{\boxepsaux}{\boxepsaux[\relax]}}
\def\boxepsaux[#1]#2#3{%
%
%   The first thing we need to do is to open the
%   PostScript file, if possible.
%
\openin\Epsffilein=\figuredirectory/#2.ps 
\ifeof\Epsffilein\message{I couldn't open \figuredirectory/#2.ps }%
\missingfigure{#2}
\else
%
%   Okay, we got it.  Now we scan lines until we find one
%   that doesn't start with a percentage sign.  We're
%   looking for the bounding box comment.
%
   {\Epsffileoktrue\Epsfbbfoundfalse
    \catcode`\%=11 \catcode`\\=11
    \catcode`\{=11 \catcode`\}=11
    \catcode`\$=11 \catcode`\^=11
    \catcode`\&=11 \catcode`\#=11
    \catcode`\~=11 \catcode`\_=11
    \loop
       \read\Epsffilein to \Epsffileline
       \ifeof\Epsffilein\Epsffileokfalse\else
%
%   Now we check to make sure the first character is a % sign,
%   and that the rest are `%BoundingBox:' if necessary.
%
          \expandafter\Epsfaux\Epsffileline . .\\%
       \fi
   \ifEpsffileok\repeat
   \ifEpsfbbfound
	\figboxht=\Epsfury\pspoints
	\advance\figboxht by-\Epsflly\pspoints
	\figboxwid=\Epsfurx\pspoints
	\advance\figboxwid by-\Epsfllx\pspoints
   \else
	\message{No bounding box comment in \figuredirectory/#2.ps }%
	\figboxwid=2in\figboxht=1in%
   \fi%
   \immediate\closein\Epsffilein
   \hscalefactor=1pt\vscalefactor=1pt%
   \scale{#3}%
   \scale{\globalscaling}%
   #1%
%
   \defscaled\DVIhscale\hscalefactor
   \defscaled\DVIvscale\vscalefactor
%
   \hscalefactor=-\Epsfllx\hscalefactor
   \hscalefactor=1.00375\hscalefactor%	--- 72.27/72 = TeXpoints/PSpoints
   \defscaled\DVIhoffset\hscalefactor
%
   \vscalefactor=-\Epsflly\vscalefactor
   \vscalefactor=1.00375\vscalefactor%	--- 72.27/72 = TeXpoints/PSpoints
   \defscaled\DVIvoffset\vscalefactor
%
   \llboxer{\special{psfile=\figuredirectory/#2.ps \DVIspace
		hoffset=\DVIhoffset\DVIspace
		voffset=\DVIvoffset\DVIspace
                hscale=\DVIhscale\DVIspace 
                vscale=\DVIvscale}} }%
\fi
}%
%
%   We need these for comparison purposes.
%
{\catcode`\%=11 \global\let\Epsfpar=\par
\global\let\Epsfpercent=%\global\def\Epsfbblit{%BoundingBox:}}%
%
%   This is our function that checks for `%BoundingBox:' and grabs the
%   values if they are found.
%
\long\def\Epsfaux#1#2 #3\\{\relax\ifx#1\Epsfpercent
   \def\testit{#2}\ifx\testit\Epsfbblit
      \Epsfsize #3 . . . .\\%
      \global\Epsffileokfalse
      \global\Epsfbbfoundtrue
   \fi\else\ifx#1\Epsfpar\else\global\Epsffileokfalse\fi\fi}%
%
%   Here we grab the values and stuff them in the appropriate definitions.
%
\def\Epsfsize#1 #2 #3 #4 #5\\{\global\def\Epsfllx{#1}\global\def\Epsflly{#2}%
   \global\def\Epsfurx{#3}\global\def\Epsfury{#4}}%




\catcode`\@=12 			% done with with internals

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% For backward compatability
%
% \pic file; height in inches; width in inches; caption\par
% \picsc file; ht (in); wid (in); scale; caption\par
%
% \mpic file; height in inches; width in inches; caption\par
% \mpicsc file; ht (in); wid (in); scale; caption\par
%
%%%%%%%%%%%%%%%%

\def\pic#1;#2;#3;#4\par{\picsc#1;#2;#3;1;#4\par}% file; wd; ht; caption 

\def\picsc#1;#2;#3;#4;#5\par{% file; wd; ht; scale; caption
\figbox[htb]{\boxeps{#1}{#4}%{#2in}{#3in}%
}{figure}{#1}{%
% (#1: #2x#3 sc #4) % 			Uncomment for debugging
#5}}


\def\mpic#1;#2;#3;#4\par{\mpicsc#1;#2;#3;1;#4\par}% file; wd; ht; caption 

\def\mpicsc#1;#2;#3;#4;#5\par{% file; wd; ht; scale; caption
\figbox[l]{\boxeps{#1}{#4}%{#2in}{#3in}%
}{figure}{#1}{%
% (#1: #2x#3 sc #4) % 			Uncomment for debugging
#5}}





==> AllReduce_Scheduling_INFOCOM'21/Supporting-Preambles/symbols-commands.tex <==
% !TEX root = ../Multi_Momentum_INFOCOM.tex

%\renewcommand{\thesection}{\Roman{section}}
%\renewcommand{\thesubsection}{\Roman{section}-\Alph{subsection}}
%\renewcommand{\thesubsubsection}{\Alph{subsection}.\arabic{subsubsection}}

\newcommand{\A}{\mathbf{A}}
\renewcommand{\a}{\mathbf{a}}
\newcommand{\B}{\mathbf{B}}
\newcommand{\Bt}{\mathbf{B}}
\renewcommand{\b}{\mathbf{b}}
\newcommand{\bt}{\mathbf{b}}
\renewcommand{\c}{\mathbf{c}}
\newcommand{\ct}{\widetilde{\mathbf{c}}}
%\newcommand{\C}{\mathbf{C}}
\newcommand{\Ch}{\widehat{\mathbf{C}}}
\newcommand{\D}{\mathbf{D}}
\newcommand{\Dh}{\widehat{\mathbf{D}}}
\renewcommand{\d}{\mathbf{d}}
\newcommand{\E}{\mathbf{E}}
\newcommand{\e}{\mathbf{e}}
\newcommand{\et}{\widetilde{\mathbf{e}}}
\newcommand{\f}{\mathbf{f}}
\newcommand{\F}{\mathbf{F}}
%\newcommand{\G}{\mathbf{G}}
\newcommand{\g}{\mathbf{g}}
\newcommand{\I}{\mathbf{I}}
\newcommand{\J}{\mathbf{J}}
\newcommand{\K}{\mathbf{K}}
\newcommand{\M}{\mathbf{M}}
\newcommand{\m}{\mathbf{m}}
\newcommand{\mh}{\widehat{\mathbf{m}}}
\newcommand{\Mh}{\widehat{\mathbf{M}}}
\newcommand{\Mt}{\widetilde{\mathbf{M}}}
\newcommand{\Mb}{\overline{\mathbf{M}}}
\newcommand{\N}{\mathbf{N}}
\newcommand{\n}{\mathbf{n}}
\newcommand{\p}{\mathbf{p}}
\renewcommand{\P}{\mathbf{P}}
\newcommand{\Q}{\mathbf{Q}}
\newcommand{\q}{\mathbf{q}}
\newcommand{\R}{\mathbf{R}}
\renewcommand{\r}{\mathbf{r}}
\renewcommand{\S}{\mathbf{S}}
\newcommand{\Sh}{\widehat{\mathbf{S}}}
\newcommand{\s}{\mathbf{s}}
\renewcommand{\t}{\mathbf{t}}
\newcommand{\T}{\mathbf{T}}
\newcommand{\Th}{\widehat{\mathbf{T}}}
%\newcommand{\U}{\mathbf{U}}
\renewcommand{\u}{\mathbf{u}}
\newcommand{\V}{\mathbf{V}}
\renewcommand{\v}{\mathbf{v}}
\newcommand{\W}{\mathbf{W}}
\newcommand{\w}{\mathbf{w}}
\newcommand{\wt}{\widetilde{\mathbf{w}}}
\newcommand{\wts}{\widetilde{w}}
\newcommand{\X}{\mathbf{X}}
\newcommand{\Xh}{\widehat{\mathbf{X}}}
\newcommand{\x}{\mathbf{x}}
\newcommand{\xt}{\widetilde{\mathbf{x}}}
\newcommand{\xh}{\widehat{\mathbf{x}}}
\newcommand{\Y}{\mathbf{Y}}
\newcommand{\y}{\mathbf{y}}
\newcommand{\z}{\mathbf{z}}
\newcommand{\Z}{\mathbf{Z}}
\newcommand{\yt}{\widetilde{\mathbf{y}}}
\newcommand{\rb}{\mathbf{b}}
\newcommand{\rvec}{\mathbf{r}}
\newcommand{\0}{\mathbf{0}}
\newcommand{\1}{\mathbf{1}}
\newcommand{\Hc}{\mathbf{H}}
\newcommand{\tHc}{\widetilde{\mathbf{H}}}
\newcommand{\hHc}{\overline{\mathbf{H}}}
\newcommand{\DL}{\mathbf{DL}}
\newcommand{\mLambda}{\mathbf{\Lambda}}
\newcommand{\vlambda}{\boldsymbol{\lambda}}
\newcommand{\mOmega}{\mathbf{\Omega}}
\newcommand{\mOmegab}{\overline{\mathbf{\Omega}}}
\newcommand{\mGamma}{\mathbf{\Gamma}}
\newcommand{\mPi}{\mathbf{\Pi}}
\newcommand{\mPsi}{\mathbf{\Psi}}
\newcommand{\mPsib}{\overline{\mathbf{\Psi}}}
\newcommand{\valpha}{\mathbf{\alpha}}
\newcommand{\vpi}{\boldsymbol \pi}
\newcommand{\Sone}{\mathcal{S}}
\newcommand{\tr}{\mathrm{Tr}}
\newcommand{\new}{\mathrm{new}}
\newcommand{\net}{\mathrm{net}}
\newcommand{\link}{\mathrm{link-phy}}
\newcommand{\LL}{\mathbf{L}}
\newcommand{\Out}[1]{\mathcal{O}\left( #1 \right)}
\newcommand{\In}[1]{\mathcal{I}\left( #1 \right)}
\newcommand{\Int}[1]{\mathcal{F}\left( #1 \right)}
\newcommand{\sInt}[1]{\hat{\mathcal{F}}\left( #1 \right)}
\renewcommand{\Re}[1]{\mbox{$\mathfrak{Re} \left( #1 \right)$}}
\renewcommand{\Im}[1]{\mbox{$\mathfrak{Im} \left( #1 \right)$}}
\newcommand{\Resq}[1]{\mbox{$\mathfrak{Re}^{2} \left( #1 \right)$}}
\newcommand{\Imsq}[1]{\mbox{$\mathfrak{Im}^{2} \left( #1 \right)$}}
\newcommand{\LTM}{\langle L \rangle}
\newcommand{\con}[1]{\overline{#1}}
\newcommand{\abs}[1]{\mbox{$\lvert #1 \rvert$}}
\newcommand{\norm}[1]{\mbox{$\left\lVert #1 \right\rVert$}}
\newcommand{\dual}{$\mathbf{D}^{\mathrm{CRPBA}}$}
\newcommand{\dnet}{$\mathbf{D}^{\mathrm{CRPBA}}_{\net}$}
\newcommand{\dlink}{$\mathbf{D}^{\mathrm{CRPBA}}_{\link}$}
\newcommand{\Pwrcon}{\Omega_{+}(n)}
\newcommand{\src}[1]{\mathrm{Src}(#1)}
\newcommand{\dst}[1]{\mathrm{Dst}(#1)}
\newcommand{\rx}[1]{\mathrm{Rx}(#1)}
\newcommand{\tx}[1]{\mathrm{Tx}(#1)}
\newcommand{\Dy}{\Delta \y}
\newcommand{\Dyt}{\Delta \widetilde{\y}}
%\newcommand*\circled[1]{\tikz[baseline=(char.base)]{
%            \node[shape=circle,draw,inner sep=2pt] (char) {#1};}}
%\newcommand{\seq}[1]{\mbox{$\{ #1 \} $}}
%\newcommand{\myref}[1]{(\ref{#1})}
%\newcommand{\sd}{\mbox{$\stackrel{\Delta}{=}$}}
%\newcommand{\sci}[2]{\mbox{$#1 \times 10^{- #2}$}}
%%\newtheorem{thm}{Theorem}

\newtheorem{thm}{Theorem}
\newtheorem{cor}[thm]{Corollary}
\newtheorem{lem}[thm]{Lemma}
\newtheorem{claim}{Claim}
\newtheorem{prop}[thm]{Proposition}
\newtheorem{ex}{Example}[section]
%\theoremstyle{definition}
\newtheorem{defn}[thm]{Definition}
%\theoremstyle{remark}
\newtheorem{finalremark}[thm]{Final Remark}
\newtheorem{rem}{Remark}
\newtheorem{sol}{Solution}
\newtheorem{fact}{Fact}
%\numberwithin{equation}[section]

\newcommand{\po}{\mbox{$ \mbox{P}_{\rm out}$}}
\newcommand{\ga}{\bar{\gamma}}
\newcommand{\mtrx}[1]{\mbox{$\left[\begin{array} #1 \end{array}\right]$}}
\newcommand{\mtrxt}[1]{\mbox{$\begin{array} #1 \end{array}$}}
\newcommand{\diag}[1]{\mathrm{Diag}\left\{ #1 \right\}}
\newcommand{\diaginv}[1]{\mathrm{Diag}^{-1}\left\{ #1 \right\}}
\newcommand{\diagtran}[1]{\mathrm{Diag}^{T}\left\{ #1 \right\}}
\newcommand{\diagv}[1]{\mathrm{diag}\left\{ #1 \right\}}
\newcommand{\etal}{{\em et al. }}
\newcommand{\ind}{\mathbbm{1}}
\newcommand{\vbeta}{\boldsymbol \beta}

\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}
\algtext*{EndWhile}% Remove "end while" text
\algtext*{EndIf}% Remove "end if" text
\algtext*{EndFor}% Remove "end while" text
\algtext*{EndFunction}% Remove "end if" text
\algtext*{EndProcedure}% Remove "end while" text
%\algtext*{EndIf}% Remove "end if" text

%\newcommand{\algorithmicinitialize}{\textbf{Initialization:}}
%\newcommand{\algorithmicmainiterate}{\textbf{Main Iteration:}}
%\newcommand{\algorithmicprimal}{\textbf{Primal Newton Direction:}}
%\newcommand{\algorithmicdual}{\textbf{Dual Variables Update:}}


==> Supporting-Preambles/jackmac.tex <==
%>From snoeyink%cs.ubc.ca@cs.Technion.AC.IL Wed Nov  3 08:18:27 1993
%Received: from csmail.cs.technion.ac.il by math.tau.ac.il (5.67/math.tau-930921)
	%id AA17625; Wed, 3 Nov 93 08:18:23 +0200
%Received: from csc (csc.cs.technion.ac.il) by csmail.cs.Technion.AC.IL (4.1/3.14)
	%id AA14244; Wed, 3 Nov 93 01:19:10 IST
%Received: from csa by csc (4.1/3.14)
	%id AA24688; Wed, 3 Nov 93 01:19:48 IST
%Received: from grolsch.cs.ubc.ca by csa (4.1/3.14)
	%id AA20525; Wed, 3 Nov 93 01:11:28 IST
%Return-Path: <snoeyink@cs.ubc.ca>
%Received: from cascade.cs.ubc.ca by grolsch.cs.ubc.ca with SMTP id AA13516
  %(5.65c/IDA-1.3.5 for alon@cs.Technion.AC.IL); Tue, 2 Nov 1993 13:56:34 -0800
%Date: Tue, 2 Nov 1993 13:56:34 -0800
%From: Jack Snoeyink <snoeyink%cs.ubc.ca@cs.Technion.AC.IL>
%Message-Id: <199311022156.AA13516@grolsch.cs.ubc.ca>
%Received: by cascade.cs.ubc.ca (4.1/SMI-4.1)
	%id AA21873; Tue, 2 Nov 93 13:56:33 PST
%To: alon@cs.Technion.AC.IL
%In-Reply-To: Alon Efrat's message of Sun, 31 Oct 93 23:38:48 IST <9310312138.AA19880@csc>
%Subject: LaTex Macros
%Status: RO
%Content-Length: 19065
%X-Lines: 638
%
%
%I'm in oberwolfach w/ micha, so I';ll just send you this and answer
%your questions on it when I get back to vancouver next week...
%
    %o                                    Jack
  %_/\_.
%(')>-(`)                          snoeyink@cs.ubc.ca
%----figbox.tex----

% 12 Oct 90 LaTeX figure boxing macros  by Jack Snoeyink
%					w/ ideas from John Hershberger
%					and code from Tom Rokicki
%%%%%%%%%%%%%%%%%
% 
% This file contains two classes of macros for dealing with figures in
% Latex documents:  
%  \figbox (and its relatives) take a box containing a figure or table
%    or whatever, caption it, and either place it on the page and wrap the
%    text around it or let it float (as usual).
%  \boxeps and \boxps take encasulated or plain postscript from a file
%    and put it in a box for use by \figbox
%
%%%%%%%%%%%%%%%%
%
% The most important macro for dealing with boxes is:
%
% \figbox: caption a box as a figure or table and place it in the margin
% 	(a marginal box) or float it (a floating box).
% 	Wide marginal boxes are promoted to one column floats; wide one
% 	column floats are promoted to two column floats.
%
% Usage: \figbox [*htblr] {box} {style} {label} {caption}
%
% The optional argument default is [htb].  Other choices
%   * two column (must come first),
%   h here, t top, b bottom (as in latex),
%   l left, r right (marginal boxes that do not float)
%
% NB: Left and right marginal boxes will not overlap in height.
%
% Two column figures default to htb unless some other 
%   	options follow the *.
%   They can also be specified by style {figure*} or {table*}.
%
% box is a box containing a figure or table.
% style is the caption style {figure}, {figure*}, {table}, or {table*}.  
% label is the label assigned.
%	if empty, the figure will not be labeled.
% caption is of the form {}, {Caption} or {[short caption] Long caption},
%       where the short caption goes into the list of figures/tables.
%	if empty, the figure will not be captioned or labeled.
% 
% The lower level macro \captionbox, described much later, can be used
% to combine two or more captioned figures into a single marginal or
% floating box.
%
%%%%%%%%%%%%%%%%
%
% options defined by macros are: \captionstyle \boxcaptionstyle
% \maxfigfraction \figboxhang \figboxmargin 
%
% \captionstyle is executed for all floating box captions
% \boxcaptionstyle is executed for all marginal box captions.
%	Default \raggedright
% \maxfigfraction is the maximum fraction of a column that can be taken up
% 	by a marginal box before it gets converted to a float.
% 	Default .6
% dimen \figboxhang is the distance a marginal box hangs into the margin.
%	Default 0pt
% dimen \figboxmargin is the width of space between the text and a
% 	marginal box. 
%	Default .15in
%
%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%
%
% The most important macros for turning postscript into boxes are:
% 
% \boxeps: Form a box containing encapsulated postscript from a file at a
%	given scale.
% \boxps: Form a box containing postscript from a file at a given scale, 
% 	width, and height.
% 
%
% Usage: \boxeps[local commands] {file} {scale}
%	 \boxps[local commands] {file} {scale} {width} {height}
%
% The optional local commands are executed after scaling. As described
% 	below, they are useful for setting origins, non-uniform scaling, etc?
% file is the filename in the \figuredirectory and without the .ps
% 	extension.
% scale is a real number: 1 to use the drawn size.  0.9 to use 90% of
% 	drawn size.  Can be changed by local commands. (see below)
% width and height are dimensions of the box produced by \boxps.
%
%%%%%%%%%%%%%%%%
%
% options: \DVIscaling \figuredirectory \missingfigure \boxer
% local commands: \horizscale \vertscale
%
% \DVIscaling is the number the dvi to ps converter considers a unit
% 	scaling transformation.  Default: 1 for dvi2ps  --- 100 for
% 	some of Rokicki's versions of dvips.
%
% \globalscaling is the scaling applied to every picture --- useful
% 	for making double size figures for journals.  Default: 1
%
% \figuredirectory is the pathname where figure postscript files are kept.
%	Default: ./figure
%
% \missingfigure{file} is executed when the file is not found.
%	Default: \def\missingfigure#1{\hbox{Missing figure #1.ps}}
%
% \boxer is the command used by \boxps to make a box of the desired size
% 	containing the figure.  Possible commands depend on the origin of
% 	the figure, and include \llboxer \lcboxer \ulboxer and \ccboxer.
% 	(ll = lower left, ul = upper left, cc = dead center, etc.)
%	\boxer can be defined in the local commands or globally.
%
% Local commands \horizscale, and \vertscale can scale the picture
% 	horizontally and vertically by different factors.  \scale
% 	scales the picture uniformly.  Scales accumulate.
%
%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%
%
% Default options
%

\def\captionstyle{}
\def\boxcaptionstyle{\raggedright}

\def\maxfigfraction{.6}% 	--- max frac of column for marg figure

\newdimen\figboxmargin%		--- margin between text and picture
\figboxmargin = .15in

\newdimen\figboxhang%		--- amount to hang picture into margin
\figboxhang = 0pt

\def\DVIscaling{1}%		--- for dvi2ps
\def\globalscaling{1}%		--- for scaling everything
\def\figuredirectory{./figures}%--- where to find the .ps files 
\let\boxer=\llboxer%		--- default origin in lower left for non-
%				      encapsulated postscript figures

\def\missingfigure#1{\hbox{Missing figure #1.ps}}


%%%%%%%%%%%%%%%%
%
% Use latex internals
%
\catcode `\@=11
\special{! /@scaleunit 1 def }

\newbox\figurebox

\def\figbox{%	[place] box style label caption
\@ifnextchar[{\figboxaux}{\figboxaux[htb]}}

%
% Parse position parameters and try appropriate placement
%
\long\def\figboxaux[#1#2]#3#4#5#6{%	--- want left margin figure?
\writepict{{#3}{#4}{#5}{#6}}%		--- save figure if journalpicts
\setbox\figurebox\hbox{#3}%
\if l#1\tryleftbox{#4}{#5}{#6}%
\else%					--- want right margin figure?
\if r#1\tryrightbox{#4}{#5}{#6}%
\else%					--- want one or two column figure?
\if *#1\checktwocoloptions#2]{\box\figurebox}{#4*}{#5}{#6}%
\else\tryonecol[#1#2]{#4}{#5}{#6}%
\fi
\fi
\fi\ignorespaces}

%
% Try a placement; promote if too wide
%

\long\def\tryleftbox#1#2#3{%		--- does left margin figure fit?
\ifdim\wd\figurebox>\maxfigfraction\columnwidth \tryonecol[htb]{#1}{#2}{#3}%
\else\leftbox{\captionbox{\box\figurebox}{#1}{#2}{#3}}\fi}

\long\def\tryrightbox#1#2#3{%	--- does right margin figure fit?
\ifdim\wd\figurebox>\maxfigfraction\columnwidth \tryonecol[htb]{#1}{#2}{#3}%
\else\rightbox{\captionbox{\box\figurebox}{#1}{#2}{#3}}\fi}

\def\checktwocoloptions{%	--- make sure twocol has htb or p
\@ifnextchar]{\floatbox[htb}{\floatbox[}}

\long\def\tryonecol[#1]#2#3#4{%	--- does one column figure fit?
\ifdim\wd\figurebox>\columnwidth \floatbox[#1]{\box\figurebox}{#2*}{#3}{#4}%
\else\floatbox[#1]{\box\figurebox}{#2}{#3}{#4}\fi}

%
% Do the work for a floating box.
%
% \floatbox[place]{box} {style} {label} {caption}
%

\long\def\floatbox[#1]#2#3#4#5{%
\begin{#3}[#1]
\hbox to \hsize{\hfil#2\hfil}
\captionandlabel{#3}{#4}{#5}
\end{#3}
}


%
% Make a caption the width of the box with given style. 
%
%\captionbox {box} {style} {label} {[optshortcap] caption}
%
% options: \boxcaptionstyle 
%
%%%%%%%%%%%%%%%%
%
% This can be used with box commands (\hbox, \vbox, \mbox, and the like),
% along with \figbox with an empty caption, to place two or more captioned
% boxes in a single marginal or floating box.   
%
% e.g. \figbox{\hbox{
%		     \captionbox{ \boxeps{fig1}1} {figure} {f1} {a figure}
%		     \hskip 1in
%		     \captionbox{ \boxeps{tab1}1} {table} {t1} {a table}
%		    }} {figure} {ignored-label} {}
%

\long\def\captionbox#1#2#3#4{% box style label {[optshortcap] caption}
\setbox\figurebox\hbox{#1}%
\parbox[t]{\wd\figurebox}{%
\bigskip\box\figurebox
\let\captionstyle=\boxcaptionstyle
\captionandlabel{#2}{#3}{#4}
\bigskip
}}

%				--- caption and label if label is nonempty
\def\captionandlabel#1#2#3{% 	--- {style} {label} {caption}
\def\testit{#3}%
\ifx\testit\empty\else%		--- if non empty caption
\writecapt{{#1}{#2}{#3}}%	--- save for journal figs
\captypeunstarred#1*.%		--- remove optional stars
\getcaption#3\endc@ption%       --- parse the caption
\def\testit{#2}%		--- check for empty label
\ifx\testit\empty\else\label{#2}\fi
\fi}

\def\captypeunstarred#1*#2.{%	--- remove two-column star from style
\def\@captype{#1}}

%
% Parse the caption of the form {caption} or {[short] long caption} 
%

\def\getcaption{\@ifnextchar[{\getcaptwo}{\getcapone}}
\long\def\getcapone#1\endc@ption{\caption[#1]%
{\def\baselinestretch{1}\Large\normalsize\captionstyle\ignorespaces #1}}
\long\def\getcaptwo[#1]#2\endc@ption{\caption[#1]%
{\def\baselinestretch{1}\Large\normalsize\captionstyle\ignorespaces #2}}

%
% Do the right thing with an already captioned marginal box
%
% \leftbox{box}
% \rightbox{box}
%
% options: \figboxmargin \figboxhang \figuredirectory

\newdimen\figboxht
\newcount\figboxn


\newcount\figboxlines%		--- picture height in number of lines
\newdimen\figboxwid%		--- picture width

\newif\ifisleftbox

\long\def\leftbox#1{%
\setbox\figurebox\hbox{#1}\global\isleftboxtrue
\startmarginbox
\vadjust{\smash{\rlap{\hskip\hsize\hskip\figboxhang
\llap{\raise.7\baselineskip\box\figurebox\hskip\rightskip}}}}%
\endmarginbox%
}

\long\def\rightbox#1{%
\setbox\figurebox\hbox{#1}\global\isleftboxfalse
\startmarginbox
\smash{\llap{\raise.7\baselineskip\box\figurebox\hskip\figboxmargin}}%
\endmarginbox%
}

\def\startmarginbox{%
\ifvmode\passpict\let\endmarginbox=\indent
\else\message{WARNING: marginbox in not in vmode}\hfilneg\ \passpict
\let\endmarginbox=\relax\fi
%
\figboxht=\dp\figurebox%	 actual height
\advance\figboxht by 1.3\baselineskip% round up
\vskip\figboxht\penalty-300\vskip-\figboxht% filbreak trick
\divide\figboxht by\baselineskip%      how many lines?
\global\figboxlines=\figboxht
%
\global\figboxwid=\wd\figurebox
\global\advance\figboxwid by \figboxmargin
\global\advance\figboxwid by -\figboxhang
\setmypar\noindent}
%

%
% Useful macros
%
% for lengthening (and shortening) picture space
%
\def\addlines#1{\global\advance\figboxlines by #1\myparshape}
\def\zerolines{\origpar\global\figboxlines=0\myparshape}

%
% for passing any marginal figures
%
\def\passpict{\par\ifnum\figboxlines>1\vskip\figboxlines\baselineskip
\zerolines\fi}

\def\emptybox#1#2{\hbox to #1{\vbox to #2{\vss}\hss}}

%%%%%%%%%%%%%%%%%%%%%
%\par hacking  
% We define our own version of Tex's \par and tell Latex it is the original

\global\let\origpar=\@@par%	--- Latex's saved version of Tex's \par
\global\let\dopar=\origpar
\global\def\@@par{\dopar}
\@setpar{\dopar}

\def\setmypar{\global\let\dopar=\mypar
\global\prevgraf=0\myparshape}

\def\mypar{\origpar\global\advance\figboxlines by -\prevgraf%
\global\prevgraf=0\myparshape}

\def\myparshape{\relax%
\ifnum\figboxlines>1\theparshape \else
\global\hangindent=0pt\global\hangafter=1%  these sometimes get restored...
\global\let\dopar=\origpar\fi}

\def\theparshape{%
\ifisleftbox\global\hangindent=-\figboxwid 
\else\global\hangindent=\figboxwid \fi
\global\hangafter=-\figboxlines \global\advance\hangafter by 1%
}


%%%%%%%%%%%%%%%%
%
%  Macros to make the list of figures and captions used by journals
%
%  To use, execute \journalpicts{scalefactor} at the beginning of the
%  file.  All figbox figures and tables will be written to a .pic file
%  and all captions to a .cap file.  On \enddocument, these files are
%  read in and the lists of figures and captions are produced.
%  
%  For non-english versions, or to add other types of floats, the
%  macro \definefnum should be changed.
%

\def\definefnum#1{%		--- ugly latex hacking to get the
%		 			right figure/table name 
\def\fnum@figure{Figure \ref{#1}}%
\def\fnum@table{Table \ref{#1}}%
\def\fnum@code{Algorithm \ref{#1}}%
}

\def\writepict#1{}
\def\writecapt#1{}

%%%%%%%%%%%%%%%%
% \journalpicts{globalscalefactor} writes all pictures and captions to
% 	files and modifies \enddocument to read these files and
% 	produce lists of enlarged figures and of captions
% 

\def\journalpicts#1{% 		global scale factor
\newwrite\pictfile
\newwrite\captfile
%
\openout\pictfile\jobname.pic
\openout\captfile\jobname.cap
%
\gdef\writepict##1{\unexpandedwrite\pictfile{\doit##1}}%
\gdef\writecapt##1{\unexpandedwrite\captfile{\doit##1}}%
%
\global\let\ENDdocument=\enddocument
\gdef\enddocument{\DOjournalpicts{#1}\ENDdocument}
}

%
%	generate enlarged figures 1 per page and list captions
%
\def\DOjournalpicts#1{{%
\def\writepict##1{}\closeout\pictfile
\def\writecapt##1{}\closeout\captfile
\@fileswfalse%			--- turn off toc, lof, and so on.
%
\onecolumn
\def\globalscaling{#1}
\def\doit##1##2##3##4{%		--- print a picture on blank page
%					{box}{style}{label}{caption}
\figboxaux[t]{\hss##1\hss}{##2}{}{}%
\vspace*{1in}
\definefnum{##3}%		--- use Figure \ref{label} or Table \ref{label}
\captionandlabel{##2}{}{##4}
\clearpage}%
%
\input\jobname.pic
%
\def\doit##1##2##3{%		--- print caption
%					{style}{label}{caption}
\definefnum{##2}%		--- use Figure \ref{label} or Table \ref{label}
\captionandlabel{##1}{}{##3}}%
%
\raggedright\let\captionstyle=\raggedright
\def\@makecaption##1##2{##1: ##2\par}%  --- Be sure captions aren't centered
%
\input\jobname.cap
}}%				--- to be followed by \enddocument



%%%%%%%%%%%%%%%%
%
%  Box macros
%
%%%%%%%%%%%%%%%%
%
% \boxeps[local commands] {file} {scale}
%
% options \DVIscaling \figuredirectory \scale \horizscale \vertscale
% \missingfigure \globalscaling
%
% \boxps[local commands] {file} {scale} {width} {height}
%
% \scale \horizscale \vertscale 

%
%  Various `boxers' --- which one is used depends on where the origin
%  of the picture is.  If you are using the bounding boxes of
%  encapsulated postscript, just use the default \llboxer.  Otherwise,
%  you have to figure out where the origin is and set \boxer appropriately.
%

\def\llboxer#1{\vbox to \figboxht{\vfil\hbox to \figboxwid{#1\hfill}}}
\def\lcboxer#1{\vbox to \figboxht{\vfil\hbox to \figboxwid{\hfill#1\hfill}}}
\def\oldboxer#1{\vbox to \figboxht{\vfil
		      \hbox to \figboxwid{\hfill\llap{#1\hskip4.25in}\hfill}}}
\def\ulboxer#1{\vbox to \figboxht{\hbox to \figboxwid{#1\hfill}\vfil}}
\def\ccboxer#1{\vbox to \figboxht{\vfil
			\hbox to \figboxwid{\hfill#1\hfill}\vfil}}

% a macro to strip the pt off a dimension
%
{\catcode`\p=12\catcode`\t=12
\gdef\removedimen#1pt{#1}}

\def\defscaled#1#2{#2=\DVIscaling#2%
\xdef#1{\expandafter\removedimen\the#2}}

\def\DVIspace{ }
\newdimen\hscalefactor
\newdimen\vscalefactor

\def\scale#1{\horizscale{#1}\vertscale{#1}}
\def\horizscale#1{\hscalefactor=#1\hscalefactor\figboxht=#1\figboxht}
\def\vertscale#1{\vscalefactor=#1\vscalefactor\figboxwid=#1\figboxwid}

%%%%%%%%%%%%%%%%
%

\def\boxps{%
\@ifnextchar[{\boxpsaux}{\boxpsaux[\relax]}}

\def\boxpsaux[#1]#2#3#4#5{%
{\figboxwid#4\figboxht#5\hscalefactor=1pt\vscalefactor=1pt%
\scale{#3}%
\scale{\globalscaling}%
#1%
\defscaled\DVIhscale\hscalefactor
\defscaled\DVIvscale\vscalefactor
\boxer{\special{psfile=\figuredirectory/#2.ps \DVIspace
		hscale=\DVIhscale\DVIspace 
		vscale=\DVIvscale}}}%
}


%%%%%%%%%%%%%%%%
% The following is from tex/inputs/epsf.tex by Tom Rokicki
% with slight modifications by Jack Snoeyink.
%
%   Written by Tomas Rokicki of Radical Eye Software, 29 Mar 1989.
%
%   Include an ecapsulated postscript graphic.
%   Works by finding the bounding box comment.
%
\newread\Epsffilein
\newif\ifEpsffileok
\newif\ifEpsfbbfound

\newdimen\pspoints
\pspoints=1in
\divide\pspoints by 72


\def\boxeps{%
\@ifnextchar[{\boxepsaux}{\boxepsaux[\relax]}}
\def\boxepsaux[#1]#2#3{%
%
%   The first thing we need to do is to open the
%   PostScript file, if possible.
%
\openin\Epsffilein=\figuredirectory/#2.ps 
\ifeof\Epsffilein\message{I couldn't open \figuredirectory/#2.ps }%
\missingfigure{#2}
\else
%
%   Okay, we got it.  Now we scan lines until we find one
%   that doesn't start with a percentage sign.  We're
%   looking for the bounding box comment.
%
   {\Epsffileoktrue\Epsfbbfoundfalse
    \catcode`\%=11 \catcode`\\=11
    \catcode`\{=11 \catcode`\}=11
    \catcode`\$=11 \catcode`\^=11
    \catcode`\&=11 \catcode`\#=11
    \catcode`\~=11 \catcode`\_=11
    \loop
       \read\Epsffilein to \Epsffileline
       \ifeof\Epsffilein\Epsffileokfalse\else
%
%   Now we check to make sure the first character is a % sign,
%   and that the rest are `%BoundingBox:' if necessary.
%
          \expandafter\Epsfaux\Epsffileline . .\\%
       \fi
   \ifEpsffileok\repeat
   \ifEpsfbbfound
	\figboxht=\Epsfury\pspoints
	\advance\figboxht by-\Epsflly\pspoints
	\figboxwid=\Epsfurx\pspoints
	\advance\figboxwid by-\Epsfllx\pspoints
   \else
	\message{No bounding box comment in \figuredirectory/#2.ps }%
	\figboxwid=2in\figboxht=1in%
   \fi%
   \immediate\closein\Epsffilein
   \hscalefactor=1pt\vscalefactor=1pt%
   \scale{#3}%
   \scale{\globalscaling}%
   #1%
%
   \defscaled\DVIhscale\hscalefactor
   \defscaled\DVIvscale\vscalefactor
%
   \hscalefactor=-\Epsfllx\hscalefactor
   \hscalefactor=1.00375\hscalefactor%	--- 72.27/72 = TeXpoints/PSpoints
   \defscaled\DVIhoffset\hscalefactor
%
   \vscalefactor=-\Epsflly\vscalefactor
   \vscalefactor=1.00375\vscalefactor%	--- 72.27/72 = TeXpoints/PSpoints
   \defscaled\DVIvoffset\vscalefactor
%
   \llboxer{\special{psfile=\figuredirectory/#2.ps \DVIspace
		hoffset=\DVIhoffset\DVIspace
		voffset=\DVIvoffset\DVIspace
                hscale=\DVIhscale\DVIspace 
                vscale=\DVIvscale}} }%
\fi
}%
%
%   We need these for comparison purposes.
%
{\catcode`\%=11 \global\let\Epsfpar=\par
\global\let\Epsfpercent=%\global\def\Epsfbblit{%BoundingBox:}}%
%
%   This is our function that checks for `%BoundingBox:' and grabs the
%   values if they are found.
%
\long\def\Epsfaux#1#2 #3\\{\relax\ifx#1\Epsfpercent
   \def\testit{#2}\ifx\testit\Epsfbblit
      \Epsfsize #3 . . . .\\%
      \global\Epsffileokfalse
      \global\Epsfbbfoundtrue
   \fi\else\ifx#1\Epsfpar\else\global\Epsffileokfalse\fi\fi}%
%
%   Here we grab the values and stuff them in the appropriate definitions.
%
\def\Epsfsize#1 #2 #3 #4 #5\\{\global\def\Epsfllx{#1}\global\def\Epsflly{#2}%
   \global\def\Epsfurx{#3}\global\def\Epsfury{#4}}%




\catcode`\@=12 			% done with with internals

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% For backward compatability
%
% \pic file; height in inches; width in inches; caption\par
% \picsc file; ht (in); wid (in); scale; caption\par
%
% \mpic file; height in inches; width in inches; caption\par
% \mpicsc file; ht (in); wid (in); scale; caption\par
%
%%%%%%%%%%%%%%%%

\def\pic#1;#2;#3;#4\par{\picsc#1;#2;#3;1;#4\par}% file; wd; ht; caption 

\def\picsc#1;#2;#3;#4;#5\par{% file; wd; ht; scale; caption
\figbox[htb]{\boxeps{#1}{#4}%{#2in}{#3in}%
}{figure}{#1}{%
% (#1: #2x#3 sc #4) % 			Uncomment for debugging
#5}}


\def\mpic#1;#2;#3;#4\par{\mpicsc#1;#2;#3;1;#4\par}% file; wd; ht; caption 

\def\mpicsc#1;#2;#3;#4;#5\par{% file; wd; ht; scale; caption
\figbox[l]{\boxeps{#1}{#4}%{#2in}{#3in}%
}{figure}{#1}{%
% (#1: #2x#3 sc #4) % 			Uncomment for debugging
#5}}




